A Systematic Mapping Study on Architectural Approaches to Software Performance Analysis

Software architecture is the foundation of a system's ability to achieve various quality attributes, including software performance. However, there lacks comprehensive and in-depth understanding of why and how software architecture and performance analysis are integrated to guide related future research. To fill this gap, this paper presents a systematic mapping study of 109 papers that integrate software architecture and performance analysis. We focused on five research questions that provide guidance for researchers and practitioners to gain an in-depth understanding of this research area. These questions addressed: a systematic mapping of related studies based on the high-level research purposes and specific focuses (RQ1), the software development activities these studies intended to facilitate (RQ2), the typical study templates of different research purposes (RQ3), the available tools and instruments for automating the analysis (RQ4), and the evaluation methodology employed in the studies (RQ5). Through these research questions, we also identified critical research gaps and future directions, including: 1) the lack of available tools and benchmark datasets to support replication, cross-validation and comparison of studies; 2) the need for architecture and performance analysis techniques that handle the challenges in emerging software domains; 3) the lack of consideration of practical factors that impact the adoption of the architecture and performance analysis approaches; and finally 4) the need for the adoption of modern ML/AI techniques to efficiently integrate architecture and performance analysis.

==> RQ-3-P1.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=1.9\columnwidth]{figures/RQ-3-Purpose-1.png}
    \caption{Classical Processes of Model-based Prediction Studies}
    \label{fig:prediction}
\end{figure*}

\paragraph{\textbf{Purpose 1: Model-based Prediction: }} Figure~\ref{fig:prediction} shows the general workflow of the studies for \textit{Model-based Prediction}. These studies usually conduct three steps for performance prediction: 1) \textit{Model-Extraction}, where an architecture model of the investigated system is extracted from the software configuration management (SCM) system; 2) \textit{Model-Annotation}, where additional performance related information, such as conditional branches or iteration loops, is annotated to the architectural model to generate an ``annotated meta-model";  3) \textit{Model-Transformation}, where the ``annotated meta-model'' are transformed into predictive performance models by means of model-to-model transformation; and finally 4) \textit{Model-Solution}, where the performance models are given to the solving tools, e.g. \textit{SHARPE}~\cite{jalali2011new}, to get the predicted performance metrics such as response time, throughput, and resource utilization. 

\textbf{Step 1: Model Extraction:} The architecture models are usually obtained in two different ways: 1) the available architecture/design models from the software design phase~\cite{yasaweerasinghelage2018predicting, reussner2016modeling, hauck2011ginpex, brosig2012modeling, groenda2012improving, trubiani2011detection}, or 2) the reverse-engineered architecture/design models from a system implementation~\cite{brosig2011automated, park2006design, trubiani2013model, moscato2007software}. In the former, the architecture/design models are manually built with a lot of time and effort in the software design phase, especially for large and complex real-world systems~\cite{brosig2011automated}. However, the availability of high-quality architecture/design models of a system is not always guaranteed. Therefore, the latter approach automatically reverse-engineers the architecture/design model from the implementation of a system. For example, \textit{Java2PCM} extracts component-level control flow from Java code, and automatically builds \textit{Palladio Component Model (PCM)} ~\cite{kappler2008towards}. Krogmann \textit{et al.} extracts behavior architecture models with the combined analysis of the run-time bytecode and static bytecode~\cite{krogmann2010using}. 
%To predict the performance for a completed system, many prior studies proposed automated methods for the extraction of architecture models. These automated model extraction methods include: 1) extraction of the application architecture that refers to the set of components and connections between components that are effectively used during operation; 2) extraction of performance related control flow inside the components, e.g. probabilities of different call paths; and 3) extraction of external service calls, e.g. a service is called multiple times by an external loop~\cite{brosig2009automated, brosig2011automated}. There are several existing reverse engineering tools that can extract architecture from a completed system. For example, \textit{Java2PCM} extracts component-level control flow from Java code and automatically builds \textit{Palladio Component Model (PCM)} ~\cite{kappler2008towards}. Krogmann \textit{et al.} presented a comprehensive approach for reverse engineering that extracts behavior architecture models from run-time bytecode counts as well as static bytecode analysis~\cite{krogmann2010using}.
Different studies extract different types of architecture models, as listed in Table~\ref{tbl: arch-model}. The extracted architecture models are in three types: %Subsequently, the model annotation and model integration are also different depending on the type of architectural model being used. Based on the different architecture models, we further categorized this group of studies into three sub-types. 

\begin{itemize}
    \item Behavioral Model: In some studies, the researchers capture the high-level architecture of a system by emphasizing the dynamic behavior of the system. This could be the collaborations among system objects, the internal state changes of objects, and the interactions among objects during system operation, etc.. More specifically, as listed from row 1 to row 3 in Table~\ref{tbl: arch-model}, the \textit{UML Sequence Diagram}, the \textit{UML Activity Diagram}, and the \textit{UML Use Case Diagram} are often used as the behavioral architecture model of a system. 
    \item Component Model: In some studies, the researchers capture the high-level architecture of a system as its fundamental building blocks and the structural connections among them. In other words, this type of models captures a system as a set of components and connectors. As shown in Table~\ref{tbl: arch-model} from row 4 to row 6, the \textit{Palladio Component Model}, the \textit{UML Component Diagram}, and the \textit{UML Deployment Diagram} are used as the component architecture model of a system. 
    \item Hybrid Model: In some studies, the researchers capture the high-level architecture of a system by simultaneously capturing the system components and their behavior interactions. Compared to the above two models, this type combines both system behavioral and component information. As shown in the last two rows in Table~\ref{tbl: arch-model}, the \textit{Probability Matrix} and \textit{Architectural Description Language} are often used as the hybrid architecture model of a system. The \textit{Probability Matrix} represents the different system behaviors on the rows and the components on the columns, while the cells capture the interactions between system behaviors and components. While the  \textit{Architectural Description Language} captures the behavioral specifications on system components and their interactions in a formal modeling language.
\end{itemize}

 
 

\begin{table*}[h!]
\small
\setlength{\tabcolsep}{12pt}
\caption{Architectural Models}
\begin{tabulary}{\textwidth}{@{}*1*{L}*3{L}@{}}
 \hline
Arch Model & Type & Description & Reference(s)  \\ [0.5ex] 
 \hline\hline
UML Sequence Diagram & Behavioral Model & It shows the sequence of messages exchanged between the objects needed to carry out the functionality of the scenario. & \cite{mani2011towards, li2016evaluating, du2015evolutionary, balsamo2004model, babar2004comparison, arcelli2013software, di2004compositional, park2006design, arcelli2015control, wu2015exploring, cortellessa2006software, trubiani2013model, das2004computing, arcelli2019exploiting}  \\ \midrule
UML Activity Diagram & Behavioral Model & It is a graphical representations of workflows of step wise activities and actions with support for choice, iteration and concurrency & \cite{de2008rup, balsamo2005performance, noorshams2014enriching} \\ \midrule
UML Use Case Diagram & Behavioral Model & It describes a system’s functional requirements in terms of use cases that enable you to relate what you need from a system to how the system delivers on those needs. & \cite{eskenazi2004analysis, di2004compositional, balsamo2005performance} \\ \midrule
Palladio Component Model (PCM) & Component Model & It is a domain specific modeling language to describe component-based software architectures. & \cite{brosig2011automated, yasaweerasinghelage2018predicting, hauck2011ginpex, brosig2012modeling, trubiani2011detection, martens2010automatically, kapova2010performance} \\ \midrule
UML Component Diagram & Component Model  & It shows a set of components and their relationships that illustrates the static implementation view of a system. & \cite{di2004compositional, eramo2012performance, cortellessa2006software, arcelli2019exploiting}  \\ \midrule
UML Deployment Diagram & Component Model  & It shows a set of nodes and their relationships that illustrates the static deployment view of an architecture. & \cite{arcelli2019exploiting, balsamo2005performance}\\ \midrule
%Descartes Meta Model (DMM) & Annotated Meta-Model & It is A novel a new meta-model for run-time quality of service and resource management in virtualized service infrastructures. & \cite{eismann2019integrating, eismann2018modeling, brosig2012modeling} \\ \midrule
Probability Matrix & Hybrid Model & It is a matrix that clarifies that one task or request with what probability enters from clients to components, or transfers from one component to other components. & \cite{jalali2011new, zhang2010improving, sharma2005architecture} \\ \midrule
Architecture Description Language (ADL) & Hybrid Model & It is a modeling language that captures the behavioral specifications of the components and their interactions that comprise the system architecture. & \cite{xu2006evaluating, cortellessa2012enabling, balsamo2004experimenting} \\
 %Event Execution Graph & & \cite{li2016evaluating}
 [1ex] 
 \hline
\end{tabulary}
\label{tbl: arch-model}
\end{table*}

%we summarized three classical processes of model-driven performance prediction. The major difference of these processes are their exploitation of architectural models. 

%\textbf{Classical Path 1) Behavior-based Architectural Models:} As shown in Figure~\ref{fig:prediction} path 2), \textit{Classical Process 2} starts from the construction of the \textit{Behavior Models}, which is shown as the top three rows on Table~\ref{tbl: arch-model}. These models emphasizes the dynamic behavior of the system by showing collaborations among objects and changes to the internal states of object, and represent the object interactions during operation.  

\textbf{Step 2: Model Annotation: } The extracted architecture models are further annotated with additional information to prepare for the following-up performance analysis and prediction. The annotation process differs mostly based on the type of architectural model. 

The \textit{Behavior Model} are annotated with quantitative information based on performance related requirements, such as service load, timing specifications, logical and physical resources, concurrency and scheduling, software and hardware infrastructure. \textitcolor{red}{In xxx out of xxx studies relying on behavior models}, the annotation process for the \textit{Behavior Models} is usually supported by two existing tools, \textit{UML/SPT (\textcolor{red}{add full name as explanation})}~\cite{di2004compositional, balsamo2005performance,cortellessa2006software} and \textit{MARTE(\textcolor{red}{add full name as explanation})}~\cite{arcelli2019exploiting, eramo2012performance}. As an example, in the case study of \cite{brosig2011automated}, \textit{UML/SPT} derives a list of call paths among the components (i.e. external service calls), and annotated the call paths with information such as the mean value of branch probability and loop iteration number. As a result, the annotated meta-model has both internal resource demanding behavior that is represented by the \textit{UML Sequence Diagram}, and the external service calls information. \textit{MARTE} is regarded as an extension of \textit{UML/SPT} tool. It focuses on real-time performance analysis and can work for real-world industrial subjects~\cite{demathieu2008first}. 
%Both tools can annotate if a component is either basic (i.e. atomic, contains not child component), or composite (i.e. contains several child component), as well as the interactions between the components. 
%\textit{UML/SPT} annotates the quantitative information directly in the UML diagrams. For example, in the case study of \cite{brosig2011automated}, it reveals that a loop is \textit{``either executed two times or ten times, each with a probability of 50\%''}. This tool annotates this information at the interactions, i.e. links, between the relevant components. 

The \textit{Component Models}, on the other hand, are usually annotated with behavioral information. For example, \textit{Palladio Component Model} is usually annotated with behavioral information through the technique, namely \textit{RDSEFF}~\cite{brosig2014quantitative}. \textit{RDSEFF} annotates the internal behavior for each component, such as the frequency that the services are called under different workload intensity~\cite{brosig2009automated}. 

The annotation process for the \textit{Hybrid Models} is more complicated. For example, in study \cite{jalali2011new}, a \textit{Probability Matrix}, as shown on Figure~\ref{fig:matrix}, is proposed to clarify the probability that one task/request enters from clients to components, from components to other components or completed and finally exits from the system. Its row and column by index zero represent clients, and 1 to n indexes represent existing components in software system. The number of each cell represents the probability . The annotation process of the \textit{Probability Matrix} is the \textit{Markov Process}, which calculates the future probability based on the most recent value for each cell~\cite{zhang2010improving}. 

\begin{figure}[ht]
  \centering
  \includegraphics[width=\columnwidth]{figures/matrix.png}  
  \caption{Example of Probability Matrix}
  \label{fig:matrix}
\end{figure}

\textbf{Step 3: Model Transformation: } The annotated meta-model are then transformed into different executable performance models as shown on Table~\ref{tbl: perf-model} . \textcolor{red}{Need more formal description of the two main types of perf-models, and explain each main type has their extensions, and what additional capabilities are these extensions provide.}


The model transformation methods are based on graph transformation techniques that transform a diagram document into a tree format~\cite{balsamo2004model}. For example, the \textit{XML Metadata Interchange (XMI)} is a commonly used transformation technique, whose input is UML diagram and output is a tree representing the corresponding \textit{Layered Queuing Network} model~\cite{bray2000extensible}. There are other transformation techniques, such as \textit{PCM2SimuCom} and \textit{PCM2QPN}~\cite{brosig2014quantitative}. \textit{PCM2SimuCom} is a model-to-text transformation method that map \textit{Palladio Component Model (PCM)} into Java code. This code is loaded by the \textit{PCM's} reference solver, namely \textit{SimuCom}, and executed during a simulation run. \textit{PCM2QPN} is use to transform \textit{PCM} to \textit{Queuing Petri Net (QPN)}, which is good at modeling hardware contention and scheduling strategies. Different model transformation techniques lead to different accuracy and efficiency for model-based prediction. For example, in \textit{PCM} model transformation techniques, as we mentioned before, \textit{PCM2SimuCom} has higher accuracy but lower time efficiency, compared to \textit{PCM2QPN}.
\begin{table*}[h!]
\small
\setlength{\tabcolsep}{12pt}
\caption{Performance Models}
\begin{center}
\begin{tabular}{ |c|c|c|c| } 
\hline
Perf Type & Description & Extension  & Reference \\
\hline
\multirow{3}{3em}{Queuing Network} & \multirow{3}{20em}{A network of queues where user or transitions (represented as \textit{customers}) queue for system resources (represented as \textit{service centers}).} & Product Form Queuing Network  & \cite{jalali2011new, sharma2005architecture, zhang2010improving}   \\ \cline{3-4}
& &  Layered Queuing Network &  \cite{mani2011towards, arcelli2013software, di2004compositional, arcelli2015control, wu2015exploring, cortellessa2006software, das2004computing, martens2010automatically} \\ \cline{3-4}
& & Extended Queueing Network  & \cite{pooley2010cpasa, trubiani2011detection, eramo2012performance}  \\ \cline{1-4}
\multirow{3}{3em}{Petri Net} & \multirow{3}{20em}{A directed bipartite graph, in which nodes represent transitions (i.e. events that may occur, represented by bars) and places (i.e. conditions, represented by circles).} & Queuing Petri Net & \cite{eismann2019integrating} \\ \cline{3-4}
&  & Colored Petri Net  & \cite{xu2006evaluating}  \\  \cline{3-4}
&  & Stochastic Petri Net  & \cite{gokhale2006performance} \\
\hline
\end{tabular}
\end{center}
\label{tbl: perf-model}
\end{table*}

\begin{comment}
\begin{table*}[h!]
\small
\setlength{\tabcolsep}{12pt}
\caption{Performance Models}
\begin{tabulary}{\textwidth}{c c c c c}
 \hline
Perf Model & Description & Sub-Type & Description &  Reference(s)\\ [0.5ex] 
 \hline\hline
\multirow{3}{*}{Queuing Network} & \multirow{3}{*}{A network of queues where user or transitions (represented as \textit{customers} queue for system resources (represented as \textit{service centers}.} &  \\ \midrule
Product Form Queuing Network & A queueing network model that have a simple closed for expression of the stationary state distribution that allows to define efficient algorithms to evaluate average performance measure. & \cite{jalali2011new, sharma2005architecture, zhang2010improving} \\ \midrule
Layered Queuing Network & A queueing network model where the service time for each job at each service node is given by the response time and those service times in turn may also be determined by further nested networks. & \cite{mani2011towards, arcelli2013software, di2004compositional, arcelli2015control, wu2015exploring, cortellessa2006software, das2004computing, martens2010automatically} \\ \midrule
Extended Queueing Network &  & \cite{pooley2010cpasa, trubiani2011detection, eramo2012performance} \\ \midrule
Queueing Petri Net  & \todo{Find its definition from the related papers.} & \cite{eismann2019integrating} \\ \midrule
Colored Petri Net   & \todo{Find its definition from the related papers.} & \cite{xu2006evaluating} \\ \midrule
Stochastic Petri Net  & \todo{Find its definition from the related papers.} & \cite{gokhale2006performance} \\ \midrule
Monte Carlo Simulation  & \todo{Find its definition from the related papers.} & \cite{trubiani2013model} \\ 
 \hline
\end{tabulary}
\label{tbl: perf-model}
\end{table*}
\end{comment}


\textbf{Step 4: Model Solution:} The performance models are solved by analytical means or by simulation to obtain performance metrics of interest, typically response time, throughput, and resource utilization~\cite{arcelli2015assisting}. The performance model solver can either be a commercial tool like \textit{SHARPE}~\cite{sahner2012performance} and \textit{SimuCom}~\cite{becker2009palladio}, or self-developed approaches such as a bunch of Eclipse Plugins developed by Meire, \textit{et al.}~\cite{meier2010automated}, namely \textit{SimQPN}, \textit{LQSim}, and \textit{LQNS}. 
%For example, in the case study of \cite{jalali2011new}, performance model \textit{PFQN} is given to \textit{SHARPE} to get the throughput of the whole system for the number range of clients determined by the user. 

%Next, the \textit{Static Structural Models} are supposed to be annotated with behavioral information. For example, in the current most commonly used component-based architectural model, \textit{Palladio Component Model (PCM)}, for each service that a component provides, the service's internal behavior is modeled using \textit{Resource-Demanding Service Effect Specifications (RDSEFF)}, that captures the control flow and resource consumption of the service depending on its input parameters passed upon invocation~\cite{brosig2012modeling}.

%These behavioral models are usually annotated with additional information to execute performance analysis, such as probabilistic branches and loop iterations. There are two commonly used tools in the annotation step, namely \textit{UML SPT (Schedulability, Performance and Time Specification) Profile} and \textit{MARTE Profile}. The \textit{UML SPT Profile} allows the specification of quantitative information directly in the UML model~\cite{di2004compositional, balsamo2005performance,cortellessa2006software}.
%The other is \textit{MARTE Profile}. This specification of a UML profile adds capabilities to UML for model-driven development of Real Time and Embedded Systems (in short, MARTES). This extension, provides support for specification, design, and verification/validation stages. Thus, this new profile is intended to replace the existing \textit{UML SPT Profile}~\cite{arcelli2019exploiting, eramo2012performance}.

%After the annotation step, \textit{``the approach can be easily integrated into standard-compliant performance modeling tool, allowing the same software model to be analyzed with different performance models''}~\cite{balsamo2005performance}.

%Finally, to predict the performance metrics, the annotated meta-model would be integrated with different performance models that represent the performance aspects of a software system as input for analytical solvers. The performance models describe how system operations use resources, and how resource contention affects operations. Such models are solved to obtain performance metrics of interest, typically response time, throughput, and utilization~\cite{arcelli2015assisting}. The most commonly used performance models are related to queueing networks, including \textit{Product Form Queueing Network}~\cite{jalali2011new, sharma2005architecture}, \textit{Layered Queueing Network}~\cite{mani2011towards, arcelli2013software, di2004compositional, arcelli2015control, wu2015exploring, cortellessa2006software, das2004computing, martens2010automatically}, and \textit{Extended Queueing Network}~\cite{pooley2010cpasa, trubiani2011detection, eramo2012performance}. A queueing network model is a a collection of service centers representing the system resources that provide service to a collection of customers that represent the users~\cite{balsamo2000product}. More than half of the \textit{Model-based Prediction} studies used queueing network models. It have been proved that queueing network model is a powerful and versatile tool for system performance evaluation and prediction. Other widely-used performance model is \textit{Place/Transition Net (Petri Net)}~\cite{eismann2019integrating, xu2006evaluating, gokhale2006performance}. \textit{Petri Net} is a directed bipartite graph, in which nodes represent transitions (i.e. events that may occur, represented by bars) and places (i.e. conditions, represented by circles).~\cite{balsamo2004model}. The directed arcs describe which places are pre and/or post conditions for which transitions, which is signified by arrows. Also, several \textit{Stochastic Process Algebra (SPA)} models have been proposed in order to describe and analyze the performance properties of software specifications~\cite{balsamo2004model, trubiani2013model, sharafi2010analytical}. The advantage of \textit{SPA} is that they allow the integration of functional and nonfunctional aspects and provide a unique reference model for software specification and performance. 
%Furthermore, a few prior studies built \textit{Simulation Models} whose structure and input parameters are derived from UML diagrams~\cite{kang2006performance, eskenazi2004analysis, yasaweerasinghelage2018predicting, park2006design, becker2013performance}. \textit{Simulation Model} is based on the assumptions about the real system's behavior.






%\paragraph{\textbf{Classical Path 2) Component Architecture Models: }} As shown in Figure~\ref{fig:prediction} path 3), \textit{Classical Process 3} starts from the construction of the \textit{Structural Models}, which is shown as the row 4, 5, and 6 on Table~\ref{tbl: arch-model}. These component-based architectural models can be constructed by mature existing tools, such as \textit{Palladio Workbench}~\cite{yasaweerasinghelage2018predicting}, or in pre-processing modules in the proposed approach, such as \textit{GINPEX}~\cite{hauck2011ginpex}. 

%Next, the \textit{Static Structural Models} are supposed to be annotated with behavioral information. For example, in the current most commonly used component-based architectural model, \textit{Palladio Component Model (PCM)}, for each service that a component provides, the service's internal behavior is modeled using \textit{Resource-Demanding Service Effect Specifications (RDSEFF)}, that captures the control flow and resource consumption of the service depending on its input parameters passed upon invocation~\cite{brosig2012modeling}. 

%The annotated meta-model, such as \textit{Descartes Meta Model (DMM)}, is for expressing and resolving parameter and context dependencies, specifically designed for use in online scenarios~\cite{brosig2012modeling}. Similarly, the final step of performance prediction is to solve the performance models that use the annotated meta-model as the input. 



%\textbf{Classical Path 3) Hybrid Architecture Models: } As shown in Figure~\ref{fig:prediction} \textit{Classical Path 3}, it starts from the construction of the \textit{Probability Matrix}~\cite{jalali2011new, zhang2010improving, sharma2005architecture}. Figure~\ref{fig:matrix} gives an example of the \textit{Probability Matrix} from the study by Jalali et al.~\cite{jalali2011new}, in which row and column by index zero represent clients, and 1 to n indexes represent existing components in software system. This matrix clarifies that one task/request with what probability enters from clients to components, from components to other components or completed and finally exits from the system~\cite{jalali2011new}. 



%It is noticeable that in \cite{jalali2011new}, the \textit{Probability Matrix} is received from the user of the system by manually entering some information such as the number of clients. But in \cite{zhang2010improving, sharma2005architecture}, the \textit{Probability Matrix} can be automatically derived by reverse engineering from the source code via the static analyzing algorithm proposed by these studies. 

%The informative annotation of this classical process is \textit{Markov process}. \textit{Markov process} is a random stochastic process whose future probabilities are determined by its most recent values~\cite{zhang2010improving}.. Thus, the system related \textit{Discrete Time Markov Chain (DTMC)} is produced~\cite{jalali2011new}. Since the \textit{Markov process} only depend on the present state and not on how the process arrived in that state, the state of the \textit{DTMC} at any time is given by the component in execution at that time~\cite{sharma2005architecture}.

%For the studies that apply \textit{Classical Path 3}, only \textit{Product Form Queueing Network (PFQN)} were used ~\cite{jalali2011new, zhang2010improving}. \textit{PFQN} has a simple closed form expression of the stationary state distribution that allow to define efficient algorithms to evaluate average performance measures~\cite{balsamo2000product}. This model is solved by the existing tool, such as \textit{SHARPE}~\cite{jalali2011new}.





% The performance models describe how system operations use resources, and how resource contention affects operations. Such models are solved to obtain performance metrics of interest, typically response time, throughput, and utilization~\cite{arcelli2015assisting}. The most commonly used performance model is queuing network, which is a collection of service centers representing the system resources that provide service to a collection of customers that represent the user~\cite{balsamo2000product}. 

==> articles.tex <==
\section{Article List}
\label{articles}

\todo{Categorize the listed articles in the format of research questions, and cancel this part.}

\textbf{1. A New Approach to Evaluate Performance of Component-Based Software Architecture (2011)}~\cite{jalali2011new}.

\purpose{1) \textbf{Predict} performance of component-based software architecture for software systems with distributed architecture. 2) \textbf{Suggest } performance optimization solutions.}

\phase{\textbf{Performance Prediction Model:} A probabilistic matrix is taken from the user and software system. The matrix clarifies that one job enter from clients to components, from components to components, or completed then exits the system.  Then, the matrix is modeled by \textit{Discrete Time Markov Chain (DTMC)}. Then, by using the \textit{DTMC} model, the amounts of visits of each component and through it the visits of each machine and connectors between machines are computed. Next, use \textit{Queueing Network} to model the system based on the data gathered previously. Finally, solving the queueing model, it outputs the bottlenecks and the required scale up is suggested. \yutong{The modeling technique belongs to reverse engineering. The entire software system is 1) automatically modeled by probabilistic matrix, 2) analyzed by \textit{DTMC}, and 3) its performance is predicted based on \textit{Queueing Network} methodology. }} 

\evaluation{The solution of the model predicts \textbf{1) throughput, 2) average response time, and 3) bottlenecks}, of the system based on various workloads. Besides performance prediction, the model can also \textbf{suggest required scale up to improve performance}. the major finding is that by increasing the number of clients, the response time will increase exponentially, but the throughput will increase logarithmically. However, the subject of this study is only an \textbf{emulated system}. }

\future{1) Adapt the model for other types of architectures, various network topologies. 2) Use various source of system.}

\textbf{2. Improving Software Performance and Reliability with an Architecture-Based Self-Adaptive Framework (2016)}~\cite{zhang2010improving}

\purpose{1) \textbf{Monitoring} and 2) \textbf{analyzing} the performance of distributed, concurrent complex software system in parallel environment. Then \textbf{3) automatically apply} the most efficient mechanism of performance improvement and reliability enhancement.}

\phase{This paper proposed a \textit{Self-Adaptive Framework for Concurrency Architectures}, e.g. cloud computing (\textit{SAFCA}). Firstly, it introduces the background of concurrency architecture alternatives, including 1) Dynamic Thread Creation (DTC): always spawns a new thread for each new traffic flow. It is simple to implement but is slow when requests burst. (2) Half-Sync/Half-Async (HS/HA): using a thread pool, aiming of simplifying programming without too much reducing performance. Async layer has higher priority as it processes newly arrived requests while a thread pool of worker threads in sync layer stored in the queuing layer. (3) Leader/Followers (LFs): the leader waits for a request from an external input. The followers stay in thread pool waiting for their turn to be the leader. LFs aims to minimize any concurrency-related overhead and to prevent race condition. Therefore, this paper designed a self-adaptive framework to advance software architecture trade-off analysis by utilizing the strengths of these three \textbf{architectural alternatives}.The framework is composed of 1) a Monitor that gathers metrics, 2) a Decider that decides if any action should be taken based on the collected data and calculated results, and 3) an Executor that informs Architecture Manager component to switchover the appropriate self-adaptive policy. To improve perforamance, when there is a sudden burst of requests and it is currently using HS/HA, the framework asks Architecture Manager to send new requests to DTC queue. After the queue length falls below the threshold, the Manager sends new requests back to the initial HS/HA queus. To improve reliability, it switches from HS/HA to LFs in case of a failure. \yutong{SAFCA can be used in 1) \textbf{Monitoring} and 2) \textbf{Executing} phases of distributed concurrent systems, such as cloud computing. In general, this approach is for solving an \textit{inefficiency under special cases} problem for a \textit{multi-threaded, concurrent system}.}}

\evaluation{They tested SAFCA on an \textbf{emulated} multi-tier system. The evaluation of experimental results showed that SAFCA has a better resource usage than an HS/HA only system and a DTC only system , and is also more quickly to bursty demands and had far fewer packet losses. In other words, SAFCA is flexible to dynamically allocate software resources, including \textbf{(1) response time; (2) message loss ratio; (3) queue length; (4) arrival rate; (5) number of threads currently running.(6) Request Drop Ratio; (7) throughput; (8) thread pool utilization; (9) CPU utilization}. This study also concerned \textbf{reliability}. }

\future{There are four major areas for future research: 1) Further improve the efficiency of the adaptive policies for different workloads and scenarios, based on performance-knowledge base by Woodside et al.~\cite{woodside2007future}; 2) investigate more different control mechanisms; 3) Integrate our proposed framework with an architecture-generic model, e.g., Rainbow~\cite{garlan2009software} ; 4) A fourth research direction is to investigate power management or energy savings with different architecture alternatives}

\textbf{3. Some experiments with the performance of LAMP architecture (2005)}~\cite{ramana2005some}. 

\purpose{Performance \textbf{1) monitoring} and \textbf{2) comparison}.}

\phase{This short paper investigated the performance of the Linux+Apache+MySQL+PHP (LAMP) architecture by several experiments. They found that (1) C performs about 400 times faster than PHP in case of computing intensive functions such as Fibonacci. (2) Performance of MySQL can be improved by eliminating the connection overhead. (3) The maximum throughput is around 26 connections per second.(4) Linux is faster than Windows for the website. In general, this study \textbf{compares} different architecture \textbf{design} for a \textbf{toy project}, based on \textbf{dynamic profiling}.}

\evaluation{Tested \textbf{toy project} of a website with different languages and various operating systems. \textbf{(1) response time; (2) throughput.} were measured.}

\future{1) increase the validity of results, 2) perform the analysis on more applications. }

\textbf{4. Integrating Statistical Response Time Models in Architectural Performance Models (2019 ICSA)}~\cite{eismann2019integrating}.

\purpose{\textbf{1) Performance prediction} by modeling software systems using classical queuing theory and statistical response time models in parallel. \textbf{2) Enabling faster model solution}, compared to traditional performance models while retaining their ability to predict previously unseen scenarios.}

\phase{This paper is quite similar to be an extension of \textit{"A New Approach to Evaluate Performance of Component-Based Software Architecture"}~\cite{jalali2011new}. The statistical response time model (SRTM) can only predict scenarios for which training data is available. The architectural performance model (APM) describe performance-relevant aspects of software architectures and execution environments allowing to evaluate different usage profiles as well as system deployment and configuration options. The generic meta-modeling approach extends component-based performance models with the ability to describe a component or sub-systems as a statistical response time model in parallel to the traditional description. They developed an algorithm to extract statistical response time models from run-time monitoring data extracted from the training data for the regression and introduce an approach to transform architectural performance models containing statistical response time models to an extended \textbf{QPN}. 

Generally speaking, this approach 
}



==> lrsrefs.tex <==
\RequirePackage{filecontents}



==> lrsrefs_before_2013.tex <==
@article{naddaf2013performance,
  title={Performance modeling and analysis of software architectures specified through graph transformations},
  author={Naddaf, Mahdi Rahimi and Rafe, Vahid},
  journal={Computing and Informatics},
  volume={32},
  number={4},
  pages={797--826},
  year={2013}
}

@article{krogmann2010using,
  title={Using genetic search for reverse engineering of parametric behavior models for performance prediction},
  author={Krogmann, Klaus and Kuperberg, Michael and Reussner, Ralf},
  journal={IEEE Transactions on Software Engineering},
  volume={36},
  number={6},
  pages={865--877},
  year={2010},
  publisher={IEEE}
}

@article{barbierato2011defining,
  title={Defining formalisms for performance evaluation with SIMTHESys},
  author={Barbierato, Enrico and Gribaudo, Marco and Iacono, Mauro},
  journal={Electronic Notes in Theoretical Computer Science},
  volume={275},
  pages={37--51},
  year={2011},
  publisher={Elsevier}
}

@inproceedings{tawhid2011automatic,
  title={Automatic derivation of a product performance model from a software product line model},
  author={Tawhid, Rasha and Petriu, Dorina C},
  booktitle={2011 15th international software product line conference},
  pages={80--89},
  year={2011},
  organization={IEEE}
}

@inproceedings{hauck2010automatic,
  title={Automatic derivation of performance prediction models for load-balancing properties based on goal-oriented measurements},
  author={Hauck, Michael and Happe, Jens and Reussner, Ralf H},
  booktitle={2010 IEEE International Symposium on Modeling, Analysis and Simulation of Computer and Telecommunication Systems},
  pages={361--369},
  year={2010},
  organization={IEEE}
}

@article{kapova2010systematic,
  title={Systematic refinement of performance models for concurrent component-based systems},
  author={Kapov{\'a}, Lucia and Becker, Steffen},
  journal={Electronic Notes in Theoretical Computer Science},
  volume={264},
  number={1},
  pages={73--90},
  year={2010},
  publisher={Elsevier}
}

@article{gaudel2011ada,
  title={An ada design pattern recognition tool for aadl performance analysis},
  author={Gaudel, Vincent and Singhoff, Frank and Plantec, Alain and Rubini, St{\'e}phane and Dissaux, Pierre and Legrand, J{\'e}r{\^o}me},
  journal={ACM SIGAda Ada Letters},
  volume={31},
  number={3},
  pages={61--68},
  year={2011},
  publisher={ACM New York, NY, USA}
}

@inproceedings{kwon2013mantis,
  title={Mantis: Automatic performance prediction for smartphone applications},
  author={Kwon, Yongin and Lee, Sangmin and Yi, Hayoon and Kwon, Donghyun and Yang, Seungjun and Chun, Byung-Gon and Huang, Ling and Maniatis, Petros and Naik, Mayur and Paek, Yunheung},
  booktitle={2013 USENIX Annual Technical Conference (USENIX ATC 13)},
  pages={297--308},
  year={2013}
}

@inproceedings{alhaj2013traceability,
  title={Traceability links in model transformations between software and performance models},
  author={Alhaj, Mohammad and Petriu, Dorina C},
  booktitle={International SDL Forum},
  pages={203--221},
  year={2013},
  organization={Springer}
}

@inproceedings{brosig2011automated,
  title={Automated extraction of architecture-level performance models of distributed component-based systems},
  author={Brosig, Fabian and Huber, Nikolaus and Kounev, Samuel},
  booktitle={Proceedings of the 26th IEEE/ACM International Conference on Automated Software Engineering},
  pages={183--192},
  organization={IEEE},
   year={2011}
}

@inproceedings{arcelli2012antipattern,
  title={Antipattern-based model refactoring for software performance improvement},
  author={Arcelli, Davide and Cortellessa, Vittorio and Trubiani, Catia},
  booktitle={Proceedings of the 8th international ACM SIGSOFT conference on Quality of Software Architectures},
  pages={33--42},
  year={2012}
}

@inproceedings{sharafi2010analytical,
  title={An analytical model for performance evaluation of software architectural styles},
  author={Sharafi, Sayed Mehran and Ghazvini, Golnaz Aghaee and Emadi, Sima},
  booktitle={2010 2nd International Conference on Software Technology and Engineering},
  volume={1},
  pages={V1--394},
  year={2010},
  organization={IEEE}
}

@inproceedings{jalali2011new,
  title={A New Approach to Evaluate Performance of Component-Based Software Architecture},
  author={Jalali, Seyed Saber and Rashidi, Hassan and Nazemi, Eslam},
  booktitle={2011 UKSim 5th European Symposium on Computer Modeling and Simulation},
  pages={451--456},
  year={2011},
  organization={IEEE}
}

@inproceedings{mani2013propagation,
  title={Propagation of incremental changes to performance model due to SOA design pattern application},
  author={Mani, Nariman and Petriu, Dorina C and Woodside, Murray},
  booktitle={Proceedings of the 4th ACM/SPEC International Conference on Performance Engineering},
  pages={89--100},
  year={2013},
  organization={ACM}
}

@inproceedings{koziolek2011peropteryx,
  title={PerOpteryx: automated application of tactics in multi-objective software architecture optimization},
  author={Koziolek, Anne and Koziolek, Heiko and Reussner, Ralf},
  booktitle={Proceedings of the 7th international ACM Sigsoft Conference on Quality of Software Architectures},
  pages={33--42},
  year={2011},
  organization={ACM}
}

@inproceedings{von2011performance,
  title={Performance simulation of runtime reconfigurable component-based software architectures},
  author={Von Massow, Robert and Van Hoorn, Andr{\'e} and Hasselbring, Wilhelm},
  booktitle={European Conference on Software Architecture},
  pages={43--58},
  year={2011},
  organization={Springer}
}

@inproceedings{berardinelli2010performance,
  title={Performance modeling and analysis of context-aware mobile software systems},
  author={Berardinelli, Luca and Cortellessa, Vittorio and Di Marco, Antinisca},
  booktitle={International Conference on Fundamental Approaches to Software Engineering},
  pages={353--367},
  year={2010},
  organization={Springer}
}

@inproceedings{wert2013supporting,
  title={Supporting swift reaction: Automatically uncovering performance problems by systematic experiments},
  author={Wert, Alexander and Happe, Jens and Happe, Lucia},
  booktitle={2013 35th International Conference on Software Engineering (ICSE)},
  pages={552--561},
  year={2013},
  organization={IEEE}
}

@inproceedings{barbierato2012perfbpel,
  title={PerfBPEL: A graph-based approach for the performance analysis of BPEL SOA applications},
  author={Barbierato, Enrico and Iacono, Mauro and Marrone, Stefano},
  booktitle={6th International ICST Conference on Performance Evaluation Methodologies and Tools},
  pages={64--73},
  year={2012},
  organization={IEEE}
}

@article{happe2010parametric,
  title={Parametric performance completions for model-driven performance prediction},
  author={Happe, Jens and Becker, Steffen and Rathfelder, Christoph and Friedrich, Holger and Reussner, Ralf H},
  journal={Performance Evaluation},
  volume={67},
  number={8},
  pages={694--716},
  year={2010},
  publisher={Elsevier}
}

@inproceedings{gambi2010model,
  title={Model-driven web engineering performance prediction with layered queue networks},
  author={Gambi, Alessio and Toffetti, Giovanni and Comai, Sara},
  booktitle={International Conference on Web Engineering},
  pages={25--36},
  year={2010},
  organization={Springer}
}

@article{martens2011monolithic,
  title={From monolithic to component-based performance evaluation of software architectures},
  author={Martens, Anne and Koziolek, Heiko and Prechelt, Lutz and Reussner, Ralf},
  journal={Empirical Software Engineering},
  volume={16},
  number={5},
  pages={587--622},
  year={2011},
  publisher={Springer}
}

@article{geetha2011framework,
  title={Framework for hybrid performance prediction process model: use case performance engineering approach},
  author={Geetha, D Evangelin and Kumar, TV Suresh and Kanth, K Rajani},
  journal={ACM SIGSOFT Software Engineering Notes},
  volume={36},
  number={3},
  pages={1--15},
  year={2011},
  publisher={ACM New York, NY, USA}
}

@inproceedings{brosig2012modeling,
  title={Modeling parameter and context dependencies in online architecture-level performance models},
  author={Brosig, Fabian and Huber, Nikolaus and Kounev, Samuel},
  booktitle={Proceedings of the 15th ACM SIGSOFT symposium on Component Based Software Engineering},
  pages={3--12},
  year={2012}
}

@article{garousi2010experience,
  title={Experience and challenges with UML-driven performance engineering of a Distributed Real-Time System},
  author={Garousi, Vahid},
  journal={Information and Software Technology},
  volume={52},
  number={6},
  pages={625--640},
  year={2010},
  publisher={Elsevier}
}

@inproceedings{cortellessa2010digging,
  title={Digging into UML models to remove performance antipatterns},
  author={Cortellessa, Vittorio and Di Marco, Antinisca and Eramo, Romina and Pierantonio, Alfonso and Trubiani, Catia},
  booktitle={Proceedings of the 2010 icse workshop on quantitative stochastic models in the verification and design of software systems},
  pages={9--16},
  year={2010}
}

@inproceedings{zulkipli2013empirical,
  title={An empirical study on performance evaluation of parallel architecture for web application services},
  author={Zulkipli, Nurul Huda Nik and Idris, Norazlan},
  booktitle={2013 IEEE Symposium on Computers \& Informatics (ISCI)},
  pages={216--221},
  year={2013},
  organization={IEEE}
}

@inproceedings{rathfelder2012workload,
  title={Workload-aware system monitoring using performance predictions applied to a large-scale e-mail system},
  author={Rathfelder, Christoph and Becker, Stefan and Krogmann, Klaus and Reussner, Ralf},
  booktitle={2012 Joint Working IEEE/IFIP Conference on Software Architecture and European Conference on Software Architecture},
  pages={31--40},
  year={2012},
  organization={IEEE}
}

@inproceedings{huber2010performance,
  title={Performance modeling in industry: a case study on storage virtualization},
  author={Huber, Nikolaus and Becker, Steffen and Rathfelder, Christoph and Schweflinghaus, Jochen and Reussner, Ralf H},
  booktitle={Proceedings of the 32nd ACM/IEEE International Conference on Software Engineering-Volume 2},
  pages={1--10},
  year={2010}
}

@inproceedings{wrzosk2012applying,
  title={Applying NAF for performance analysis: Performance analysis of SOA systems using LQN models},
  author={Wrzosk, Arkadiusz},
  booktitle={2012 Military Communications and Information Systems Conference (MCC)},
  pages={1--8},
  year={2012},
  organization={IEEE}
}

@inproceedings{khan2010performance,
  title={A Performance modeling framework incorporating cost efficient deployment of collaborating components},
  author={Khan, Razib Hayat and Heegaard, Poul E},
  booktitle={Proceedings of the 2nd International Conference on Software Technology and Engineering},
  pages={331--340},
  year={2010},
  organization={IEEE}
}

@article{litoiu2013performance,
  title={A performance evaluation framework for web applications},
  author={Litoiu, Marin and Barna, Cornel},
  journal={Journal of Software: Evolution and Process},
  volume={25},
  number={8},
  pages={871--890},
  year={2013},
  publisher={Wiley Online Library}
}

@article{arcelli2013software,
  title={Software model refactoring based on performance analysis: better working on software or performance side?},
  author={Arcelli, Davide and Cortellessa, Vittorio},
  journal={Formal Engineering approaches to Software Components and Architectures},
  pages={33--47}
  year={2013},
  
}

@Run Time},
  pages={31--40},
  year={2010},
  organization={IEEE}
}

@inproceedings{kapova2010performance,
  title={Performance-driven stepwise refinement of component-based architectures},
  author={Kapova, Lucia and Buhnova, Barbora},
  booktitle={Proceedings of the 2nd International Workshop on the Quality of Service-Oriented Software Systems},
  pages={1--7},
  year={2010}
}

@inproceedings{eramo2012performance,
  title={Performance-driven architectural refactoring through bidirectional model transformations},
  author={Eramo, Romina and Cortellessa, Vittorio and Pierantonio, Alfonso and Tucci, Michele},
  booktitle={Proceedings of the 8th international ACM SIGSOFT conference on Quality of Software Architectures},
  pages={55--60},
  year={2012},
  organization={ACM}
}

@inproceedings{perez2010performance,
  title={Performance aware open-world software in a 3-layer architecture},
  author={Perez-Palacin, Diego and Merseguer, Jos{\'e} and Bernardi, Simona},
  booktitle={Proceedings of the 1st Joint WOSP/SIPEW International Conference on Performance Engineering},
  pages={49--56},
  year={2010},
  organization={ACM}
}

@inproceedings{becker2013performance,
  title={Performance analysis of self-adaptive systems for requirements validation at design-time},
  author={Becker, Matthias and Luckey, Markus and Becker, Steffen},
  booktitle={Proceedings of the 9th international ACM Sigsoft conference on Quality of software architectures},
  pages={43--52},
  year={2013}
}

@inproceedings{trubiani2013model,
  title={Model-based performance analysis of software architectures under uncertainty},
  author={Trubiani, Catia and Meedeniya, Indika and Cortellessa, Vittorio and Aleti, Aldeida and Grunske, Lars},
  booktitle={Proceedings of the 9th international ACM Sigsoft conference on Quality of software architectures},
  pages={69--78},
  year={2013}
}

@inproceedings{groenda2012improving,
  title={Improving performance predictions by accounting for the accuracy of composed performance models},
  author={Groenda, Henning},
  booktitle={Proceedings of the 8th international ACM SIGSOFT conference on Quality of Software Architectures},
  pages={111--116},
  year={2012},
  organization={ACM}
}

@inproceedings{hauck2011ginpex,
  title={Ginpex: deriving performance-relevant infrastructure properties through goal-oriented experiments},
  author={Hauck, Michael and Kuperberg, Michael and Huber, Nikolaus and Reussner, Ralf},
  booktitle={Proceedings of the 7th International ACM SIGSOFT Conference on Quality of Software Architectures},
  pages={53--62},
  year={2011},
  organization={ACM}
}

@inproceedings{tribastone2010performance,
  title={Performance prediction of service-oriented systems with layered queueing networks},
  author={Tribastone, Mirco and Mayer, Philip and Wirsing, Martin},
  booktitle={International Symposium On Leveraging Applications of Formal Methods, Verification and Validation},
  pages={51--65},
  year={2010},
  organization={Springer}
}

@inproceedings{camara2013evolving,
  title={Evolving an adaptive industrial software system to use architecture-based self-adaptation},
  author={C{\'a}mara, Javier and Correia, Pedro and De Lemos, Rog{\'e}rio and Garlan, David and Gomes, Pedro and Schmerl, Bradley and Ventura, Rafael},
  booktitle={2013 8th International Symposium on Software Engineering for Adaptive and Self-Managing Systems (SEAMS)},
  pages={13--22},
  year={2013},
  organization={IEEE}
}

@inproceedings{trubiani2011detection,
  title={Detection and solution of software performance antipatterns in palladio architectural models},
  author={Trubiani, Catia and Koziolek, Anne},
  booktitle={Proceedings of the 2nd ACM/SPEC International Conference on Performance engineering},
  pages={19--30},
  year={2011}
}

@inproceedings{heger2013automated,
  title={Automated root cause isolation of performance regressions during software development},
  author={Heger, Christoph and Happe, Jens and Farahbod, Roozbeh},
  booktitle={Proceedings of the 4th ACM/SPEC International Conference on Performance Engineering},
  pages={27--38},
  year={2013}
}

==> proposal.tex <==
\section{For Lu's Proposal}
\label{proposal}

\subsection{Purpose}

\paragraph{1. Performance prediction:} These studies predict the performance indices, such as speed of execution, resource utilization, and throughput, without having to really execute the software system, i.e. dynamic profiling, in early stages of software life-cycles. This type has two sub-types. Firstly, in some studies, it gives suggestions on how to use more efficient architectural solutions based on different use case scenarios, e.g~\cite{jalali2011new, pooley2010cpasa, du2015evolutionary, yasaweerasinghelage2018predicting, eramo2012performance, perez2010performance, martens2010automatically, kapova2010performance}. Secondly, in other studies, it simply predicts the performance of system(s) under different scenarios without giving suggestions, e.g.~\cite{eismann2019integrating, brosig2011automated, brosig2014quantitative, kang2006performance, li2016evaluating, de2008rup, balsamo2004model, eismann2018modeling, sharafi2010analytical, eskenazi2004analysis, arcelli2019exploiting, di2004compositional, park2006design, hauck2011ginpex, brosig2012modeling, groenda2012improving, wu2015exploring, sharma2005architecture, moreno2008performance, balsamo2005performance, cortellessa2006software, moscato2007software, trubiani2013model, perez2014dealing, noorshams2014enriching, brosig2011automated, brebner2012experiences, balsamo2004experimenting, pagliari2019extent}.

\paragraph{2. Experimental comparison of performance of different architectural solution: } These studies use dynamically profiling process to monitor the runtime-time performance of different architectural solution, based on different use case / scenarios. For example, \cite{ramana2005some, xu2006evaluating, shinozaki2006performance, babar2004comparison, hill2010run, le2011state, priyadarsini2017performance, liu2011impact, xenopoulos2016big, ferreira2016peesos, taifi2015jenergy, gokhale2006performance, seelig2006performance, fioravanti2016experimental, krebs2014metrics, etxeberria2014performance, seabra2019rest, das2004computing, gupta2008architecting, menasce2008heuristic, castellanos2019measuring, ramirez2014performance}.

\paragraph{3. Self-adaptive performance improvement: } These studies proposed self-adaptive approaches/frameworks that integrate monitoring, analyzing, and execution functionalities has the potential to accommodate an ever dynamically changing environment, e.g. ~\cite{zhang2010improving, agrawal2015source, ferretti2014performance, allan2004odepack++, camara2013evolving, arcelli2015control, becker2012model, becker2013performance, guha2010balancing}.

\paragraph{4. Performance anti-pattern detection and solution: } To detect, or solve performance anti-patterns for refactoring, e.g. ~\cite{mani2011towards, cortellessa2012enabling, arcelli2013software, arcelli2019exploiting, trubiani2011detection, rudzki2006performance, wert2014automatic, arcelli2012antipattern}.

\paragraph{5. Performance issue categorization: } These studies aim to collect and categorize performance problems based on their root cause, solution, and so on. For example, ~\cite{zhao2020performance, arcelli2015assisting}.

\subsection{Life-Cycle Phase}

\paragraph{1. Requirement verification/specification: } \cite{pooley2010cpasa, kang2006performance, de2008rup, perez2010performance}.

\paragraph{2. Software Design:} \cite{jalali2011new, eismann2019integrating, mani2011towards, brosig2014quantitative, pooley2010cpasa, kang2006performance, li2016evaluating, du2015evolutionary, de2008rup, balsamo2004model, eismann2018modeling, sharafi2010analytical, eskenazi2004analysis, ferretti2014performance, di2004compositional, park2006design, hauck2011ginpex, groenda2012improving, sharma2005architecture, eramo2012performance, etxeberria2014performance, becker2012model, moreno2008performance, balsamo2005performance, cortellessa2006software, becker2013performance, moscato2007software, trubiani2013model, das2004computing, perez2014dealing, perez2010performance, noorshams2014enriching, brosig2011automated, castellanos2019measuring, brebner2012experiences, balsamo2004experimenting, pagliari2019extent, ramirez2014performance, martens2010automatically, kapova2010performance}.

\paragraph{3. Run-time:} \cite{zhang2010improving, ramana2005some, brosig2011automated, xu2006evaluating, shinozaki2006performance, babar2004comparison, eismann2018modeling, sharafi2010analytical, hill2010run, le2011state, priyadarsini2017performance, liu2011impact, xenopoulos2016big, agrawal2015source, arcelli2019exploiting, ferreira2016peesos, taifi2015jenergy, yasaweerasinghelage2018predicting, allan2004odepack++, gokhale2006performance, seelig2006performance, camara2013evolving, hauck2011ginpex, fioravanti2016experimental, brosig2012modeling, arcelli2015control, wu2015exploring, krebs2014metrics, rudzki2006performance, etxeberria2014performance, becker2012model, moreno2008performance, moscato2007software, trubiani2013model, seabra2019rest, gupta2008architecting, menasce2008heuristic, perez2014dealing, castellanos2019measuring, pagliari2019extent, guha2010balancing, ramirez2014performance, kapova2010performance}.

\paragraph{4. Maintenance/Testing: } \cite{cortellessa2012enabling, arcelli2013software, zhao2020performance, arcelli2015assisting, trubiani2011detection, wert2014automatic, menasce2008heuristic, castellanos2019measuring, arcelli2012antipatte}.

\paragraph{5. Software Evolution: } \cite{li2016evaluating, hauck2011ginpex}
 







==> rq-3-p1-new.tex <==
\paragraph{\textbf{Purpose 1: Model-based Prediction: }} Figure~\ref{fig:prediction} shows the general workflow of the studies for \textit{Model-based Prediction}. These studies usually conduct four steps for performance prediction: 1) \textit{Model-Acquisition}, where an architecture model of the investigated system is acquired; 2) \textit{Model-Annotation}, where the architecture model is annotated with performance-related information, such as resource demands, conditional branching probabilities, and loop iterations, to generate an ``annotated meta-model";  3) \textit{Model Transformation}, where the ``annotated meta-models'' are transformed into predictive performance models by means of model-to-model transformations; and finally 4) \textit{Model Solution}, where the performance models 
are resolved to get the predicted performance metrics such as response time, throughput, and resource utilization. 

\begin{figure*}
    \centering
    \includegraphics[width=1.9\columnwidth]{figures/rq-3-prediction.png}
    \caption{Overview of Model-based Prediction Studies}
    \label{fig:prediction}
\end{figure*}

\textbf{1) Model Acquisition: } The \textit{Model-based Prediction} starts with the architecture model acquisition. The architecture models are usually obtained in two different ways. In the first case, the architecture models are directly available and acquired from the initial architecture/design documents~\cite{yasaweerasinghelage2018predicting, reussner2016modeling, hauck2011ginpex, brosig2012modeling, groenda2012improving, trubiani2011detection}. In this case, software designer manually create the high-level architecture/design models of a system. These design documents are kept in the software configuration management systems for future reference and analysis. However, building high-quality architecture models usually requires big up-front investment in the software design phase, especially for large and complex real-world systems~\cite{brosig2011automated}. Thus, architecture design models and documentations are not always available in practice. In the second case, the architecture models are obtained through reverse engineering from a system implementation~\cite{brosig2011automated, park2006design, trubiani2013model, moscato2007software, park2006design, hauck2011ginpex, sharma2005architecture, moreno2008performance, kappler2008towards, krogmann2010using}. For example, \textit{Java2PCM} is a commonly used tool to extract a \textit{Palladio Component Model (PCM)}, detailing the component-level control flow, reverse engineered from Java code~\cite{kappler2008towards}. %Krogmann \textit{et al.} extracts behavior architecture models with the combined analysis of the run-time bytecode and static bytecode~\cite{krogmann2010using}. 

\begin{table*}[h!]
\small
\setlength{\tabcolsep}{12pt}
\caption{Architecture Models}
\begin{tabulary}{\textwidth}{@{}*2{L}*3{L}@{}}
 \hline
Arch Model & Type & Description & Reference(s)  \\ [0.5ex] 
 \hline\hline
UML Sequence Diagram & Behavioral Model & It shows the sequence of messages exchanged between the objects needed to carry out the functionality of the scenario. & \cite{mani2011towards, li2016evaluating, du2015evolutionary, balsamo2004model, babar2004comparison, arcelli2013software, di2004compositional, park2006design, arcelli2015control, wu2015exploring, cortellessa2006software, trubiani2013model, das2004computing, arcelli2019exploiting}  \\ \midrule
UML Activity Diagram & Behavioral Model & It is a graphical representations of workflows of step wise activities and actions with support for choice, iteration and concurrency & \cite{de2008rup, balsamo2005performance, noorshams2014enriching} \\ \midrule
UML Use Case Diagram & Behavioral Model & It describes a system’s functional requirements in terms of use cases that enable you to relate what you need from a system to how the system delivers on those needs. & \cite{eskenazi2004analysis, di2004compositional, balsamo2005performance} \\ \midrule
Message Sequence Chart & Behavioral Model & It is a trace language for the specification and description of the communication behaviour of system components and their environment by means of message interchange. & \cite{li2016evaluating, balsamo2004model} \\ \hline\hline
Palladio Component Model & Component Model & It is a domain specific modeling language to describe component-based software architecture with respect to static structure, deployment, allocation, resource environment, and usage profile. & \cite{brosig2011automated, yasaweerasinghelage2018predicting, hauck2011ginpex, brosig2012modeling, trubiani2011detection, martens2010automatically, kapova2010performance, das2004computing, noorshams2014enriching} \\ \midrule
UML Component Diagram & Component Model  & It shows a set of components and their relationships that illustrates the static implementation view of a system. & \cite{di2004compositional, eramo2012performance, cortellessa2006software, arcelli2019exploiting}  \\ \midrule
UML Deployment Diagram & Component Model  & It shows a set of nodes and their relationships that illustrates the static deployment view of an architecture. & \cite{arcelli2019exploiting, balsamo2005performance}\\ \hline\hline
%Descartes Meta Model (DMM) & Hybrid Model & It is A novel a new meta-model for run-time quality of service and resource management in virtualized service infrastructures. & \cite{eismann2019integrating, eismann2018modeling, brosig2012modeling} \\ \midrule
Probability Matrix & Hybrid Model & It is a matrix that clarifies that one task or request with what probability enters from clients to components, or transfers from one component to other components. & \cite{jalali2011new, zhang2010improving, sharma2005architecture} \\ \midrule
Architecture Description Language & Hybrid Model & It is a modeling language that captures the behavioral specifications of the components and their interactions that comprise the system architecture. & \cite{xu2006evaluating, cortellessa2012enabling, balsamo2004experimenting} \\
[1ex] 
 \hline
\end{tabulary}
\label{tbl: arch-model}
\end{table*}

The architecture models used for performance prediction in the reviewed studies are summarized in Table~\ref{tbl: arch-model}. In this table, we list the name (column 1), the type (column 2), a brief description (column 3) of each model, and the respective studies that rely on each model (column 4). As indicated in column 2, these architecture models can be categorized in general three types, explained following:
\begin{itemize}
    \item Behavioral Model: In some studies, the researchers capture the high-level architecture of a system by emphasizing the dynamic behavior of the system. This could be the collaborations among system objects, the internal state changes of objects, and the interactions among objects during system operation, etc.. As listed from row 1 to row 4 in Table~\ref{tbl: arch-model}, the \textit{UML Sequence Diagram}, the \textit{UML Activity Diagram}, the \textit{UML Use Case Diagram}, and the \textit{Message Sequence Chart}, are the behavioral architecture models. 
    \item Component Model: In some studies, the researchers capture the high-level architecture of a system as the fundamental building blocks and the connections among them. In other words, this type of models captures a system as a set of components, connectors, and their compositions. As shown in Table~\ref{tbl: arch-model} from row 5 to row 7, the \textit{Palladio Component Model}, the \textit{UML Component Diagram}, and the \textit{UML Deployment Diagram} are used as the structural architecture model of a system. 
    \item Hybrid Model: In some studies, the researchers capture the high-level architecture of a system by simultaneously capturing the system components and their behavioral interactions. Compared to the above two models, this type combines both system behavioral and component structure information in the model. As shown in the last three rows in Table~\ref{tbl: arch-model}, the \textit{Descartes Meta-Model}, \textit{Probability Matrix} and \textit{Architectural Description Language} are the hybrid architecture models for describing a system. The \textit{Probability Matrix} represents the different system behaviors on the rows and the components on the columns, while the cells capture the interactions between system behaviors and components. While the  \textit{Architectural Description Language} captures the behavioral specifications on system components and their interactions in a formal modeling language.
\end{itemize}

\textbf{2) Model Annotation: } Performance prediction requires additional information that are not present in the architecture models. Thus, the second step of the \textit{Model-based Prediction} process is to annotate the architecture model with performance-related data~\cite{becker2008coupled}. The annotation aims to include additional information, covering the resource demands~\cite{brosig2011automated, brosig2014quantitative, yasaweerasinghelage2018predicting, hauck2011ginpex, brosig2012modeling, groenda2012improving, moreno2008performance, martens2010automatically, kapova2010performance, noorshams2014enriching}, branching probabilities~\cite{di2004compositional, balsamo2005performance,cortellessa2006software}, input parameter characterisations~\cite{arcelli2019exploiting, eramo2012performance}, workload specifications~\cite{jalali2011new, pooley2010cpasa, yasaweerasinghelage2018predicting, eramo2012performance}, etc. 

Resource demands is the estimated required resource for finishing a process under a certain scenario, such as 



The annotation process differs based on the type of architecture model.

The \textit{Behavior Models} are annotated with quantitative information based on performance related requirements, such as service load, timing specifications, logical and physical resources, concurrency and scheduling, and software infrastructure. In 13 out of 19 studies that rely on \textit{Bahavior Models} (nearly 70\%), the model annotation process are supported by two approaches, \textit{UML-SPT}~\cite{di2004compositional, brosig2011automated, balsamo2005performance, cortellessa2006software, pooley2010cpasa, moreno2008performance, das2004computing, arcelli2015assisting, noorshams2014enriching, balsamo2004experimenting} and \textit{UML-MARTE}~\cite{arcelli2019exploiting, eramo2012performance, perez2010performance, martens2010automatically}.

\textit{UML-SPT} is the abbreviation of \textit{UML Profile for Schedulability, Performance, and Time}, which annotates performance-related information such as workload status, time intervals between requests, and execution probabilities~\cite{becker2008coupled}. For example, in study \cite{balsamo2005performance}, the software architecture is described in two type of \textit{Bahevior Models}, e.g. \textit{UML Use Case Diagram} and \textit{UML Activity Diagram}, and these diagrams are annotated according to the \textit{UML-SPT}. First, the \textit{UML-SPT} annotates the status of workload that can be either closed or open. In a closed workload, a fixed population of requests repeatedly interact with the system. In an open workload, there is an infinite stream of external requests. As shown on Figure~\ref{fig:annotated-use-case-diagram}, the actor \textit{User} is annotated as <<PAOpenLoad>>, while the actor \textit{Time} was annotated as <<PAClosedLoad>>. Furthermore, in a closed workload, after a use case is executed, there is a short delay called ``think time'' after which the use case is executed again~\cite{becker2008coupled}. Thus, below the <<PAClosedLoad>> tag, \textit{UML-SPT} annotates a ``PAextDelay'' tag that describes the ``think time'' by each completed request before the next interaction with the system. In the \textit{UML Activity Diagram}, as shown on Figure~\ref{fig:annotated-activity-diagram}, the transitions are annotated with an execution probability tag ``PAprob'', which represents the probability of taking one specific transition.

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{figures/annotated-use-case-diagram.png}
    \caption{Example of Annotated UML Use Case Diagram~\cite{balsamo2005performance}}
    \label{fig:annotated-use-case-diagram}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{figures/annotated-activity-diagram.png}
    \caption{Example of Annotated UML Activity Diagram~\cite{balsamo2005performance}}
    \label{fig:annotated-activity-diagram}
\end{figure}

\textit{UML-MARTE} is the abbreviation of \textit{UML Modeling and Analysis of Real Time and Embedded systems}. It is an extension of \textit{UML-SPT} that focuses on real-time performance analysis and can work for real-world industrial subjects~\cite{demathieu2008first}. For example, in \cite{perez2010performance}, the \textit{UML Activity Diagram} is annotate by \textit{UML-MARTE} with timing specification related information, such as time intervals between requests. 

The \textit{Component Models} are usually annotated with the parametric contracts that specify the inner behavior of a component~\cite{becker2008coupled, brosig2014quantitative, brosig2009automated}. In 9 out of 14 studies that rely on \textit{Bahavior Models} (64\%), the model annotation process are supported by \textit{Resource Demanding Service EFFect specification}, in short, \textit{RD-SEFF}~\cite{brosig2011automated, yasaweerasinghelage2018predicting, hauck2011ginpex, brosig2012modeling, trubiani2011detection, martens2010automatically, kapova2010performance, das2004computing, noorshams2014enriching}. 

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{figures/RD-SEFF.png}
    \caption{Example of Resource Demanding Service EFFect specification (RD-SEFF)~\cite{noorshams2014enriching}}
    \label{fig:RD-SEFF}
\end{figure}

\textit{RF-SEFF} reflects parametric dependencies to input parameters and the execution environment. For example, in study \cite{noorshams2014enriching}, the I/O requests of the component is annotated by \textit{RD-SEFF} with four parameters, as illustrated in Figure~\ref{fig:RD-SEFF}. The ``Request size'' specifies the I/O demand. The ``Request type'' defines either read or write. The ``Sequentiality'' is the percentage or probability of a sequential request. And the ``File set'' is the name and size of file set that the request is operating on. The need for the former two parameters is obvious, e.g. small read request and large write request is entirely different. These two parameters reflect the property of input of the component. The latter two parameters are required to estimate the impact of external execution environment, e.g. if the file set is too large to fit in the caching hierarchy. 

The annotation process for the \textit{Hybrid Models} is more complicated and may different from each other. For example, in study \cite{jalali2011new}, a \textit{Probability Matrix}, as shown on Figure~\ref{fig:matrix}, is proposed to clarify the probability that one task/request enters from clients to components, from components to other components or completed and finally exits from the system. Its row and column by index zero represent clients, and 1 to n indexes represent existing components in software system. The number of each cell represents the probability. The annotation process of the \textit{Probability Matrix} is the \textit{Markov Process}, which calculates the future probability based on the most recent value for each cell~\cite{zhang2010improving}. As a result, the annotate meta-model, a \textit{Discrete Time Markov Chain (DTMC)}, as shown in Figure~\ref{fig:DTMC}, is produced after the annotation. In the \textit{DTMC} model, the top two nodes represent the recent states, and the below nodes represent the potential derived states. The transition arrows are annotated with P (for probability) that describe the probability of one state evolves to another state. 

\begin{figure}[ht]
  \centering
  \includegraphics[width=\columnwidth]{figures/matrix.png}  
  \caption{Example of Probability Matrix~\cite{jalali2011new}}
  \label{fig:matrix}
\end{figure}

\begin{figure}[ht]
  \centering
  \includegraphics[width=\columnwidth]{figures/DTMC.png}  
  \caption{Example of Discrete Time Markov Chain (DTMC)~\cite{jalali2011new}}
  \label{fig:DTMC}
\end{figure}

\textbf{3) Model Transformation: } The annotated meta-models have to be transformed into different performance models that can be  The transformation are classified into two sub-types: model-to-model (M2M) transformation and model-to-text (M2T) transformation~\cite{becker2008coupled}. Model-to-model transformation is specified in some special languages, e.g. \textit{XML} executable by a specific transformation technique, e.g. \textit{XML Metadata Interchange (XMI)}. Model-to-text transformation is a special class of model-to-model transformations where the target model is simply an text file.

\textit{Palladio Component Model (PCM)} can be transformed into performance model by either \textit{M2M} transformation, e.g. \textit{PCM2LQN} and \textit{PCM2QPN}, or \textit{M2T} transformation ,e.g. \textit{PCM2SimuCom}~\cite{brosig2014quantitative}. \textit{PCM2SimuCom} is a model-to-text transformation, which maps \textit{PCM} into \textit{Java} code. This code is loaded by \textit{SimuCom}, which is the abbreviation of \textit{Simulation for Component-based systems}. The process of \textit{PCM2SimuCom} transformation has been fully automated as it has been compacted into \textit{Eclipse} plugins~\cite{yasaweerasinghelage2018predicting}. \textit{PCM2SimuCom} transformation is wide-used for the studies that are based on \textit{PCM} architecture model, since 5 ~\cite{martens2010automatically, brosig2011automated, yasaweerasinghelage2018predicting, brosig2014quantitative, trubiani2011detection} ot of the 9 studies that used \textit{PCM} transform the annotated architecture model by \textit{PMC2SimuCom}. \textit{PCM} can also be transformed directly into performance models. \textit{PCM2LQN} and \textit{PCM2QPN} are model-to-model transformation that is directly based on model stored in the concrete syntax as defined by \textit{XML}. Both of these two transformations use \textit{XMI} as the transformation technique, which transforms \textit{PCM} into a tree format that represents the corresponding model such as \textit{LQN} and \textit{QPN}~\cite{yasaweerasinghelage2018predicting, kapova2010performance, becker2013performance}.

The transformation from UML diagrams to performance models are also highly automated. The most wide-used UML transformation technique is \textit{Janus Transformation Language (JTL)}, which is a model-to-text transformation language that specifically suites for change propagation analyzing~\cite{eramo2012performance, eramo2012performance, li2016evaluating, de2008rup}. The \textit{JTL} transformation is written in \textit{JTL} syntax, and it has been also compacted into \textit{Eclipse} plugins~\cite{eramo2012performance}. The UML diagrams are firstly translated into \textit{Generalized Performance Interchange Format (GMPIF)} by the \textit{JTL} engine plugin. After that, the \textit{GMPIF} to performance model transformation is very similar to the model-to-model transformations e.g. \textit{PCM2LQN} and \textit{PCM2QPN}, because \textit{GMPIF} is also defined in \textit{XML}. The \textit{XMI} technique, as mentioned above, can map the elements into the performance model.

The transformation of \textit{Architectural Description Language (ADL)} into performance models is similar to UML transformations but it does not have an existing tool like \textit{JTL}. Also, because the \textit{ADL} itself is defined in syntax format language, which is similar to \textit{XML}, the \textit{XMI} can directly map the elements into the performance model, without having to translate it to meta-model such as \textit{GMPIF}~\cite{xu2006evaluating}. For the \textit{M2T} transformation of \textit{ADL}, each action state in the \textit{ADL} is translated into a simulation process~\cite{trubiani2013model}.

Since the \textit{Probability Matrix} is annotated by \textit{Markov Process} into a \textit{Discrete-Time Markov Chain (DTMC)}, which can be directly used as the input of \textit{Product Form Queuing Network}, the transformation process of such studies is neglected.  

%The transformation based on \textit{Architectural Description Language (ADL)} is firstly parsed by \textit{XMI}, because the \textit{ADL} itself is also defined in \textit{XML}. 

The output of the transformation are the predictive performance models as shown on Table~\ref{tbl: perf-model}.. The following gives a brief overview of the most important ones, i.e. \textit{Queuing Network}, \textit{Petri Nets}, and \textit{Stochastic Process Algebra}. \textit{Queuing Network} reflects both the structural and behavioral aspects of the system. Yet, \textit{Petri Nets} and \textit{Stochastic Process Algebra} tend to be more behavioral~\cite{pooley2010cpasa}. From the architecture design point of view, structural aspects are more important, making the \textit{Queuing Network} more suitable for this scope of work~\cite{balsamo2004model}.

\begin{table*}[h!]
\small
\setlength{\tabcolsep}{12pt}
\caption{Output of Model Transformation}
\begin{center}
\begin{tabular}{ |c|c|c|c| } 
\hline
Perf Type & Description & Extension  & Reference \\
\hline
\multirow{3}{4em}{Queuing Networks} & \multirow{3}{23em}{A network of queues where user or transitions (represented as \textit{customers}) queue for system resources (represented as \textit{service centers}).} & Product Form Queuing Network  & \cite{jalali2011new, sharma2005architecture, zhang2010improving}   \\ \cline{3-4}
& &  Layered Queuing Network &  \cite{mani2011towards, arcelli2013software, di2004compositional, arcelli2015control, wu2015exploring, cortellessa2006software, das2004computing, martens2010automatically, pagliari2019extent, brosig2011automated, balsamo2004experimenting} \\ \cline{3-4}
& & Extended Queueing Network  & \cite{pooley2010cpasa, trubiani2011detection, eramo2012performance}  \\ \cline{1-4}
\multirow{3}{4em}{Stochastic Petri Nets} & \multirow{3}{23em}{A directed bipartite graph that consists of a set of \textit{places} (i.e. conditions, represented by circles) and \textit{transitions} (i.e. events that may occur, represented by bars).} & Queuing Petri Net & \cite{eismann2019integrating, brosig2014quantitative} \\ \cline{3-4}
&  & Colored Petri Net  & \cite{xu2006evaluating}  \\  \cline{3-4}
&  & Generalized Stochastic Petri Net  & \cite{gokhale2006performance, li2016evaluating, moscato2007software, perez2010performance} \\ \cline{1-4}
\multirow{3}{4em}{Stochastic Process Algebra} & \multirow{2}{23em}{Abstract languages used to describe sequential behaviors which may run concurrently, and synchronizations or communications between them.} & TIPP & \cite{pooley2010cpasa, balsamo2004model} \\ \cline{3-4}
&  & EMPA  & \cite{kang2006performance}  \\  \cline{3-4}
&  & PEPA  & \cite{balsamo2004experimenting} \\ \hline\hline
\multirow{3}{4em}{Simulation Code} & \multicolumn{2}{|l|}{\multirow{3}{40em}{The programming code generated from the instances of \textit{PCM} that can be directly used for the discrete-event simulation.}} & \cite{martens2010automatically, kapova2010performance, brosig2011automated, yasaweerasinghelage2018predicting, balsamo2004model, brosig2014quantitative, becker2013performance, wu2015exploring}\\ 
& \multicolumn{2}{|l|}{} &  \\ 
& \multicolumn{2}{|l|}{} &  \\ 
\hline
\end{tabular}
\end{center}
\label{tbl: perf-model}
\end{table*}

Our findings confirms with the study by Cortellesa \textit{et al.}~\cite{cortellessa2004three} in 2004, that the \textit{Queuing Networks} are the most preferred performance models. 54\% of the \textit{Model-based Prediction} studies used \textit{Queuing Networks}. A \textit{Queuing Network} model is a collection of interacting \textit{service centers} representing system resources, and a set of \textit{jobs} representing the users sharing the resources~\cite{pagliari2019extent, becker2008coupled}.  \textit{Jobs} travel through a network of \textit{service centers} using probabilistic routes. The analytical solution of \textit{Queuing Network} predicts the average response time of the overall system, waiting times for queues, average queue length, and server utilization~\cite{becker2008coupled}. A very simple example of \textit{Queuing Network} is illustrated as Figure~\ref{fig:queuing-network}. It depicts a closed workload scenario which has been mentioned above. A delay server models the ``think time'' which is indicated by the clock at the bottom. After a processing step on the CPU, jobs either use a hard-drive (HDD) with a probability of 30\% or a network resource (NET) with a probability of 70\%.

\begin{figure}[ht]
  \centering
  \includegraphics[width=\columnwidth]{figures/queuing-network.png}  
  \caption{Example of Queuing Network~\cite{becker2008coupled}}
  \label{fig:queuing-network}
\end{figure}

A certain type of \textit{Queuing Networks}, namely \textit{Product Form Queuing Network (PFQN)}, can compute the predicted results precisely in very short time. However, the application of \textit{PFQN} is very restrictive because many realistic system, such as priority queues, is not in product form. From our observation, the \textit{PFQN} is only used to model ``Toy Projects'' that are rather simple and self-developed by developer, which we will describe in later section~\cite{jalali2011new, sharma2005architecture, zhang2010improving}. To model real-life, complicated software systems, several enhancements of \textit{Queueing Networks} exist, such as \textit{Layered Queuing Network (LQN)}~\cite{mani2011towards, arcelli2013software, di2004compositional, arcelli2015control, wu2015exploring, cortellessa2006software, das2004computing, martens2010automatically} and \textit{Extended Queuing Network (EQN)}~\cite{pooley2010cpasa, trubiani2011detection, eramo2012performance}. In \textit{LQN}, servers can issue requests to other servers during the processing of a job for their client. Software entities and hardware entities are represented as nodes in an acyclic graph. This acylic graph depicts the dependencies of node during job processing~\cite{mani2011towards, cortellessa2006software}. \textit{EQN} provides different colored highlighting spots that represents different control flow constructs like forks, branches, or backware jumps~\cite{pooley2010cpasa}. 

A \textit{Stochastic Petri Net} consists of a set of places and transitions, which are traversed by tokens~\cite{becker2008coupled, balsamo2004model}. Transitions remove and add tokens on places whenever they are active. \textit{Stochastic Petri Net} is well suited to analyze concurrent behavior and relevant properties such as deadlock freedom~\cite{xu2006evaluating, eismann2019integrating, becker2008coupled}. \textit{Generalized Stochastic Petri Net (GSPN)} is viewed as a formalism for the description of the global behavior of complex structures. It is the most basic form of \textit{Stochastic Petri Net}. \textit{GSPN} include two classes of transitions: 1) exponentially distributed timed transitions, which are used to model the random delays associated with the execution of activities; and 2) the immediate transitions, which represent the logical actions that do not consume time. Immediate transitions permits the existing of branching probabilities that are independent of timing specification~\cite{balbo2007introduction}. \textit{Colored Petri Net} provides a framework for the construction and analysis of distributed systems~\cite{xu2006evaluating}. It has the advantage of describing the behavior of the resource sharing and synchronization. \textit{Queuing Petri Net} is the combination of \textit{Queuing Network} and \textit{Colored Petri Net} that can easily model hardware contention and scheduling strategies as well as software contention, synchronization, blocking, and asynchronous processing~\cite{brosig2014quantitative}.

Several \textit{Stochastic Process Algebras} have been proposed to describe and analyze the performance properties. The advantage of using \textit{Stochastic Process Algebras} is that they allow the integration of functional and nonfunctional aspects and provide a unique reference model for software specification and performance~\cite{balsamo2004model}. Three different sub-types of \textit{Stochastic Process Algebra} were used in the selected studies, e.g. \textit{Time Processes and Performability Evaluation (TIPP)}~\cite{pooley2010cpasa, balsamo2004model}, \textit{Extended Markovian Process Algebra (EMPA)}~\cite{kang2006performance}, and \textit{Performance Evaluation Process Algebra (PEPA)} ~\cite{balsamo2004experimenting}. All of them associate with exponentially distributed random variables to actions. Besides exponential actions, passive and immediate actions are also considered~\cite{balsamo2004model}. \textit{TIPP} is suitable for describing the behavior of a system because it is achieve by the convention that a certain random distribution function is associated with every action~\cite{hermanns1994performance}. In \textit{TIPP}, each action is represented as a pair consisting of an action name and the according random distribution function. \textit{EMPA} enhances the expressiveness of classical processes algebras in two ways. First, it offers actions whose duration is exponentially distributed as well as immediate actions, hence it is useful for performance abstraction. Second, the actions are able to be parameterized by priority levels and weights, hence the prioritized choices and probabilistic choices can be implemented~\cite{bernardo1996extended}. \textit{PEPA} also extends classical process algebras by introducing probabilistic branching and the timing of transitions, but it is more automated since it has been compacted into \textit{Eclipse} plugins. 

\textbf{4) Model Solution: } Predicted performance metrics such as response time are obtained by solving the performance models. There are two different ways of solving the performance models: by simulation~\cite{martens2010automatically, noorshams2014enriching, brosig2011automated, balsamo2004experimenting, kang2006performance, yasaweerasinghelage2018predicting, becker2013performance, brosig2011automated, brosig2014quantitative, eskenazi2004analysis, park2006design, hauck2011ginpex, brosig2012modeling, groenda2012improving} and by analytical techniques~\cite{perez2010performance, das2004computing, balsamo2004experimenting, pagliari2019extent, jalali2011new, pooley2010cpasa, eramo2012performance, eismann2019integrating, xu2006evaluating, li2016evaluating, balsamo2004model, eismann2018modeling, sharafi2010analytical, di2004compositional, wu2015exploring, sharma2005architecture, moreno2008performance, balsamo2005performance, moscato2007software, trubiani2013model}. 

Simulation is an imitation of the operations of a system monitored over a period of time~\cite{pooley2010cpasa}. The advantage of simulation is the high degree of accuracy~\cite{becker2008coupled, pooley2010cpasa}. However, the disadvantage of simulation is that it is very time consuming, especially for large-scale complex systems~\cite{becker2008coupled, balsamo2004experimenting}. 6 out of 14 studies that used simulation applies \textit{SimuCom} as the simulation tool~\cite{martens2010automatically, kapova2010performance, brosig2011automated, yasaweerasinghelage2018predicting, balsamo2004model, brosig2014quantitative}. \textit{SimuCom} is the default simulator of \textit{PCM} and it is based on transformation of the \textit{PCM} instance to a process-based discrete-event simulation~\cite{brosig2014quantitative}. Another \textit{PCM} simulator, \textit{PerOpteryx}, that also takes instances of the annotated meta-model from \textit{PCM} as the input, has been compacted as a set of plugins embedded in \textit{Eclipse}~\cite{trubiani2011detection, martens2010automatically}. \textit{SimuLizar}, which was used in the study~\cite{becker2013performance}, is also an \textit{Eclipse} plugin that also takes \textit{PCM}'s meta-model as its input. \textit{SimuLizar} is a more comprehensive tool that not supports the simulation process to obtain the predicted performance metrics, but also supports the analysis for scalability, flexibility, and reliability. \textit{EventSim} is faster than \textit{SimuCom} and suites for systems with very high concurrency. In the study~\cite{wu2015exploring}, \textit{EventSim} was used to get the simulation results of a \textit{Layered Queuing Network} performance model and this study predicted the performance of a real-life open sourced project, \textit{Hadoop}. Some performance models have their specific simulation solvers. For example, \textit{LQN Simulation} is the default simulation solver for \textit{Layered Queuing Network}~\cite{eskenazi2004analysis, park2006design}, and \textit{SimQPN} is the the default simulation solver for \textit{Queing Petri Net}~\cite{brosig2014quantitative}.

Analytical solution only works for a range of performance models with very limited assumption, but solving analytically is much faster than simulation~\cite{pooley2010cpasa}. Usually, the performance models have default analytical solution tool. \textit{Symbolic Hierarchical Automated Reliability and Performance Evaluator (SHARPE)} is a very useful analytical solution tool that contains algorithms for the analysis of fault trees, acyclic series-parallel graphs, and Markov or semi-Markov models~\cite{trivedi2002sharpe}. In our selected studies, all the studies that use \textit{Product Form Queuing Network} which are produced from \textit{Discrete Time Markov Chain} use \textit{SHARPE} to provide analytical solution~\cite{jalali2011new, sharma2005architecture, zhang2010improving}. The \textit{Layered Queuing Network} has its default analytical solver named \textit{LQN Solver (LQNS)}, which provides fast numeric approximation for \textit{LQN} models~\cite{ani2011towards, di2004compositional, wu2015exploring, cortellessa2006software, martens2010automatically, pagliari2019extent, balsamo2004experimenting}. Similarly, \textit{Queuing Petri Net} has its default solver named \textit{QPN Solver}~\cite{eismann2019integrating}. \textit{GreatSPN} is a graphical user interface written in \textit{Java} language that can be used to draw \textit{Generalized Stochastic Petri Nets (GSPN)}~\cite{li2016evaluating, balsamo2004model}. It is a highly automated tool that has a rich set of graphical elements representing immediate and exponential transitions of \textit{GSPN}. The analytical solution of \textit{Stochastic Algebra Process} usually uses an efficient algorithm for state space generate to transform the algebra into a semi-Markov process~\cite{balsamo2005performance}. This approach has been implemented using the tool \textit{DSPNexpress 2000}~\cite{lindemann2000quantitative}, which supports the quantitative analysis of discrete-even stochastic processes. After that, the generalized semi-Markov model can be solved by using tools such as \textit{SHARPE}, etc. 

==> rq-3-p1-v2.tex <==
\paragraph{\textbf{Purpose 1: Model-based Prediction: }} Figure~\ref{fig:prediction} shows the general workflow of the studies for \textit{Model-based Prediction}. These studies usually conduct four steps for performance prediction: 1) \textit{Model-Acquisition}, where an architecture model of the investigated system is acquired; 2) \textit{Model-Annotation}, where the architecture model is annotated with performance-related information, such as resource demands, conditional branching probabilities, and loop iterations, to generate an ``annotated meta-model";  3) \textit{Model Transformation}, where the ``annotated meta-models'' are transformed into predictive performance models by means of model-to-model transformations; and finally 4) \textit{Model Solution}, where the performance models 
are resolved to get the predicted performance metrics such as response time, throughput, and resource utilization. 

\begin{figure*}
    \centering
    \includegraphics[width=1.9\columnwidth]{figures/rq-3-prediction.png}
    \caption{Overview of Model-based Prediction Studies}
    \label{fig:prediction}
\end{figure*}

\textbf{1) Model Acquisition: } The \textit{Model-based Prediction} starts with the architecture model acquisition. The architecture models are usually obtained in two different ways. In the first case, the architecture models are directly available and acquired from the initial architecture/design documents~\cite{yasaweerasinghelage2018predicting, reussner2016modeling, hauck2011ginpex, brosig2012modeling, groenda2012improving, trubiani2011detection}. In this case, software designer manually create the high-level architecture/design models of a system. These design documents are kept in the software configuration management systems for future reference and analysis. However, building high-quality architecture models usually requires big up-front investment in the software design phase, especially for large and complex real-world systems~\cite{brosig2011automated}. Thus, architecture design models and documentations are not always available in practice. In the second case, the architecture models are obtained through reverse engineering from a system implementation~\cite{brosig2011automated, park2006design, trubiani2013model, moscato2007software, park2006design, hauck2011ginpex, sharma2005architecture, moreno2008performance, kappler2008towards, krogmann2010using}. For example, \textit{Java2PCM} is a commonly used tool to extract a \textit{Palladio Component Model (PCM)}, detailing the component-level control flow, reverse engineered from Java code~\cite{kappler2008towards}. %Krogmann \textit{et al.} extracts behavior architecture models with the combined analysis of the run-time bytecode and static bytecode~\cite{krogmann2010using}. 

\begin{table*}[h!]
\small
\setlength{\tabcolsep}{12pt}
\caption{Architecture Models}
\begin{tabulary}{\textwidth}{@{}*2{L}*3{L}@{}}
 \hline
Arch Model & Type & Description & Reference(s)  \\ [0.5ex] 
 \hline\hline
UML Sequence Diagram & Behavioral Model & It shows the sequence of messages exchanged between the objects needed to carry out the functionality of the scenario. & \cite{mani2011towards, li2016evaluating, du2015evolutionary, balsamo2004model, babar2004comparison, arcelli2013software, di2004compositional, park2006design, arcelli2015control, wu2015exploring, cortellessa2006software, trubiani2013model, das2004computing, arcelli2019exploiting}  \\ \midrule
UML Activity Diagram & Behavioral Model & It is a graphical representations of workflows of step wise activities and actions with support for choice, iteration and concurrency & \cite{de2008rup, balsamo2005performance, noorshams2014enriching} \\ \midrule
UML Use Case Diagram & Behavioral Model & It describes a system’s functional requirements in terms of use cases that enable you to relate what you need from a system to how the system delivers on those needs. & \cite{eskenazi2004analysis, di2004compositional, balsamo2005performance} \\ \midrule
Message Sequence Chart & Behavioral Model & It is a trace language for the specification and description of the communication behaviour of system components and their environment by means of message interchange. & \cite{li2016evaluating, balsamo2004model} \\ \hline\hline
Palladio Component Model & Component Model & It is a domain specific modeling language to describe component-based software architecture with respect to static structure, deployment, allocation, resource environment, and usage profile. & \cite{brosig2011automated, yasaweerasinghelage2018predicting, hauck2011ginpex, brosig2012modeling, trubiani2011detection, martens2010automatically, kapova2010performance, das2004computing, noorshams2014enriching} \\ \midrule
Descartes Modeling Language & Component Model & It is an architecture-level modeling language for quality-of-service and resource management of modern dynamic IT systems and infrastructures. & \cite{eismann2019integrating, eismann2018modeling, brosig2012modeling} \\ \midrule
UML Component Diagram & Component Model  & It shows a set of components and their relationships that illustrates the static implementation view of a system. & \cite{di2004compositional, eramo2012performance, cortellessa2006software, arcelli2019exploiting}  \\ \midrule
UML Deployment Diagram & Component Model  & It shows a set of nodes and their relationships that illustrates the static deployment view of an architecture. & \cite{arcelli2019exploiting, balsamo2005performance}\\ \hline\hline
Probability Matrix & Hybrid Model & It is a matrix that clarifies that one task or request with what probability enters from clients to components, or transfers from one component to other components. & \cite{jalali2011new, zhang2010improving, sharma2005architecture} \\ \midrule
Architecture Description Language & Hybrid Model & It is a modeling language that captures the behavioral specifications of the components and their interactions that comprise the system architecture. & \cite{xu2006evaluating, cortellessa2012enabling, balsamo2004experimenting} \\
[1ex] 
 \hline
\end{tabulary}
\label{tbl: arch-model}
\end{table*}

The architecture models used for performance prediction in the reviewed studies are summarized in Table~\ref{tbl: arch-model}. In this table, we list the name (column 1), the type (column 2), a brief description (column 3) of each model, and the respective studies that rely on each model (column 4). As indicated in column 2, these architecture models can be categorized in general three types, explained following:
\begin{itemize}
    \item Behavioral Model: In some studies, the researchers capture the high-level architecture of a system by emphasizing the dynamic behavior of the system. This could be the collaborations among system objects, the internal state changes of objects, and the interactions among objects during system operation, etc.. As listed from row 1 to row 4 in Table~\ref{tbl: arch-model}, the \textit{UML Sequence Diagram}, the \textit{UML Activity Diagram}, the \textit{UML Use Case Diagram}, and the \textit{Message Sequence Chart}, are the behavioral architecture models. 
    \item Component Model: In some studies, the researchers capture the high-level architecture of a system as the fundamental building blocks and the connections among them. In other words, this type of models captures a system as a set of components, connectors, and their compositions. As shown in Table~\ref{tbl: arch-model} from row 5 and row 8, textit{Palladio Component Model (PCM)}, the \textit{Descartes Modeling Language (DML)}, the \textit{UML Component Diagram}, and the \textit{UML Deployment Diagram} are used as the structural architecture model of a system. 
    \item Hybrid Model: In some studies, the researchers capture the high-level architecture of a system by simultaneously capturing the system components and their behavioral interactions. Compared to the above two models, this type combines both system behavioral and component structure information in the model. As shown in the last two rows in Table~\ref{tbl: arch-model}, the \textit{Probability Matrix} and \textit{Architectural Description Language} are the hybrid architecture models for describing a system. The \textit{Probability Matrix} represents the different system behaviors on the rows and the components on the columns, while the cells capture the interactions between system behaviors and components. While the  \textit{Architectural Description Language} captures the behavioral specifications on system components and their interactions in a formal modeling language.
\end{itemize}

\textbf{2) Model Annotation: } Performance prediction requires additional information that are not present in the architecture models. Thus, the second step of the \textit{Model-based Prediction} process is to annotate the architecture model with performance-related data~\cite{becker2008coupled}. The annotation aims to include additional information, covering the branching probabilities~\cite{di2004compositional, balsamo2005performance,cortellessa2006software}, workload status~\cite{jalali2011new, pooley2010cpasa, yasaweerasinghelage2018predicting, eramo2012performance}, timing specifications~\cite{perez2010performance, arcelli2019exploiting, eramo2012performance}, scheduling policy~\cite{di2004compositional, eramo2012performance, cortellessa2006software, arcelli2019exploiting, balsamo2005performance}, and resource demands~\cite{brosig2011automated, brosig2014quantitative, yasaweerasinghelage2018predicting, hauck2011ginpex, brosig2012modeling, groenda2012improving, moreno2008performance, martens2010automatically, kapova2010performance, noorshams2014enriching}, etc. 

Branching probability represents the probability of taking one specific conditional process~\cite{balsamo2005performance}. It is related to performance because conditional process with high probability has stronger impact on performance than the process with low probability. Branching probability information can be collected by either static code analysis by analyzing the condition of activing of a process, or dynamic monitoring the count of activation~\cite{becker2008coupled}. Branching probability is usually annotated to \textit{Behavior Models} by the existing automated tool, \textit{UML Profile for Schedulability, Performance, and Time (UML-SPT)}~\cite{di2004compositional, balsamo2005performance,cortellessa2006software}. For example, in the study \cite{balsamo2005performance}, as shown on Figure~\ref{fig:annotated-activity-diagram}, the transitions are annotated with an execution probability tag, namely ``PAprob'', which represents the probability of taking one specific transition. After transmitting the job ``ACK'', there are 90\% probability to go back to the step of framework preparation, but only 10\% probability of terminating the process. Thus, when calculating the total response time and memory utilization of ``Player'' from initializing to terminating, the iteration with probability as high as 90\% is obviously supposed to be paid more attention. 

The status of workload can be either closed or open~\cite{becker2008coupled, eramo2012performance, balsamo2005performance}. In a closed workload, a fixed population of requests repeatedly interact with the system. In an open workload, there is an infinite stream of external requests. It is related to performance because if the workload status is closed, there exists a short delay namely ``think time'' after which process is executed again with a certain use case~\cite{balsamo2005performance}. Workload specification is usually annotated by the existing tool \textit{UML-SPT}, which has been mentioned above, or \textit{UML Modeling and Analysis of Real Time and Embedded systems (UML-MARTE)}, which is an extension of \textit{UML-SPT} that focuses on real-time performance analysis and can work for real-world industrial subjects~\cite{demathieu2008first}. As shown in Figure~\ref{fig:annotated-use-case-diagram} in study \cite{balsamo2005performance}, the actor \textit{User} is annotated as <<PAOpenLoad>> that represents an open workload, while the actor \textit{Time} was annotated as <<PAClosedLoad>> that represents a closed workload. Below the <<PAClosedLoad>> tag, \textit{UML-SPT} annotates a ``PAextDelay'' tag that describes the ``think time'' by each completed request before the next interaction with the system.

Timing specification information are like the time intervals between requests~\cite{perez2010performance}, the time to acquire and release a job~\cite{becker2008coupled, arcelli2019exploiting}. This is related to performance because it directly impacts on the speed of process. For example, as shown on Figure~\ref{fig:timing-specification-annotation} in the study \cite{perez2010performance}, the UML Activity Diagram is annotated with the time intervals between requests, i.e. ``interArrivalTime = 500 time units'' on the top block, by using \textit{UML MARTE}. This timing specification information indicates the requests arrive to the component with an exponential inter-arrival time, with a mean of 500 time units. 
%Similarly, in the study \cite{balsamo2005performance}, as shown on Figure~\ref{fig:scheduling-policy}, \textit{UML-MARTE} annotates <<PAschedPolicy>> tag, ``First In First Out (FIFO)'', to the \textit{UML Deployment Diagram} is for all the three active processors, i.e., a video server, a client machine, and the network. 


Scheduling policy includes ``First In First Out (FIFO)'', ``Last In First Out (LIFO)'', and ``Processor Sharing (PS)''. It is related to performance because it specifies the schedule of the jobs handled by a processor~\cite{balsamo2005performance}. For example, as shown on Figure~\ref{fig:scheduling-policy} in study \cite{balsamo2005performance}, \textit{UML-MARTE} annotates <<PAschedPolicy>> tag to the \textit{UML Deployment Diagram} is for all the three active processors: a video server, a client machine, and the network. 


Resource demands is the estimated required resource of which process jobs actively until the job is fully processed, such as the storage resource like the capacity of memory~\cite{brosig2012modeling, groenda2012improving, noorshams2014enriching}, the  number of operations per time unit need for CPU~\cite{noorshams2014enriching, brosig2012modeling, groenda2012improving, moreno2008performance, martens2010automatically, kapova2010performance}, the type and size of the external requests~\cite{brosig2014quantitative, yasaweerasinghelage2018predicting, hauck2011ginpex, noorshams2014enriching}, and I/O rate of disks~\cite{becker2008coupled, brosig2011automated, brosig2014quantitative, yasaweerasinghelage2018predicting}. It is related to performance because it models the execution environment that helps to calculate the maximum and minimum bound of estimated response time. Resource demand is usually annotated as the inner behavioral information into \textit{Component Models} by the existing technique namely \textit{Resource Demanding Service EFFect specification}, in short, \textit{RD-SEFF}~\cite{brosig2011automated, yasaweerasinghelage2018predicting, hauck2011ginpex, brosig2012modeling, trubiani2011detection, martens2010automatically, kapova2010performance, das2004computing, noorshams2014enriching}. As shown in Figure~\ref{fig:RD-SEFF} of the study \cite{noorshams2014enriching}, the business component is annotated an encapsulated I/O resource request interface by \textit{RD-SEFF}. The I/O resource request interface is comprised of four parameters , as illustrated in Figure~\ref{fig:RD-SEFF}. The ``Request size'' specifies the I/O demand. The ``Request type'' defines either read or write. The ``Sequentiality'' is the percentage or probability of a sequential request. And the ``File set'' is the name and size of file set that the request is operating on. The need for the former two parameters is obvious, e.g. small read request and large write request is entirely different. These two parameters reflect the property of input of the component. The latter two parameters are required to estimate the impact of external execution environment, e.g. if the file set is too large to fit in the caching hierarchy. 

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{figures/annotated-activity-diagram.png}
    \caption{UML Activity Diagram annotated with Branching Probability~\cite{balsamo2005performance}}
    \label{fig:annotated-activity-diagram}
\end{figure}



\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{figures/annotated-use-case-diagram.png}
    \caption{UML Use Case Diagram annotated with Workload Status~\cite{balsamo2005performance}}
    \label{fig:annotated-use-case-diagram}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{figures/timing-specification-annotation.png}
    \caption{UML Activity Diagram annotated with Timing Specification~\cite{perez2010performance}}
    \label{fig:timing-specification-annotation}
\end{figure}


\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{figures/scheduling-policy.png}
    \caption{UML Deployment Diagram annotated with Scheduling Policy~\cite{balsamo2005performance}}
    \label{fig:scheduling-policy}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{figures/RD-SEFF.png}
    \caption{Palladio Component Model annotated with Resource Demands~\cite{noorshams2014enriching}}
    \label{fig:RD-SEFF}
\end{figure}

The \textit{Model Annotation} process is highly relevant to the type of original architecture models. In our selected studies, 13 out of 19 (68\%) \textit{Model-based Prediction} studies that use \textit{Behavior Models}, are annotated branching probabilities, workload status, and timing specifications by using the existing tool \textit{UML-SPT}~\cite{di2004compositional, brosig2011automated, balsamo2005performance, cortellessa2006software, pooley2010cpasa, moreno2008performance, das2004computing, arcelli2015assisting, noorshams2014enriching, balsamo2004experimenting} and \textit{UML-MARTE}~\cite{arcelli2019exploiting, eramo2012performance, perez2010performance, martens2010automatically}. 

%All the five studies that use \textit{Structural Models} are annotated the inner behavior of a basic component, such as inner-component timing specifaction~\cite{di2004compositional, eramo2012performance, cortellessa2006software, arcelli2019exploiting, balsamo2005performance}, and processor's scheduling policy~\cite{arcelli2019exploiting, balsamo2005performance}. Since all the two \textit{Structural Models} that appeared in our selected studies are \textit{UML Diagrams}, these information are also be annotated with \textit{UML-SPT} and \textit{UML-MARTE}. 

The \textit{Component Models} are usually annotated with inner behavior information of a component~\cite{becker2008coupled, brosig2014quantitative, brosig2009automated}. As the example in Figure~\ref{fig:scheduling-policy}, the component (processor) is annotated with the job scheduling policy as ``First In First Out (FIFO)''. In 12 out of 17 (70\%) studies that use \textit{Palladio Component Model (PCM)} and \textit{Descartes Modeling Language (DML)}, the inner behavior of a component, such as internal resource comsumption~\cite{walter2015automated} is annotated by \textit{RD-SEFF}~\cite{brosig2011automated, yasaweerasinghelage2018predicting, hauck2011ginpex, brosig2012modeling, trubiani2011detection, martens2010automatically, kapova2010performance, das2004computing, noorshams2014enriching, eismann2019integrating, eismann2018modeling, brosig2012modeling}. Although both \textit{PCM} and \textit{DML} are architecture models to describe component-based systems, however, from the historic perspective, \textit{PCM} is designed for design time scenarios but \textit{DML} targets reconfiguration at run-time~\cite{walter2015automated}.Thus, \textit{DML} can be annotated with more behavioral information than internal resource consumption, such as external call paths~\cite{eismann2018modeling, eismann2019integrating}. 

The annotation process for the \textit{Hybrid Models} is more complicated. The \textit{Probability Matrix}, as shown on Figure~\ref{fig:matrix}, is proposed to clarify the probability that one task/request enters from clients to components, from components to other components or completed and finally exits from the system. Its row and column by index zero represent clients, and 1 to n indexes represent existing components in software system. The number of each cell represents the probability. The annotation process of the \textit{Probability Matrix} is a \textit{Markov Process}, which calculates the future probability based on the most recent value for each cell~\cite{zhang2010improving}. As a result, the annotate meta-model, a \textit{Discrete Time Markov Chain (DTMC)}, as shown in Figure~\ref{fig:DTMC}, is produced after the annotation. In the \textit{DTMC} model, the top two nodes represent the recent states, and the below nodes represent the potential derived states. The transition arrows are annotated with P (for probability) that describe the probability of one state evolves to another state. The annotation process for \textit{Architecture Description Language (ADL)} prefers more detailed information in timing specification. For example, in \cite{cortellessa2012enabling, balsamo2004experimenting}, the \textit{ADL} is annotated with the mean value of the possible delays between the activities and the synchronization constrains of the scheduling policy of processor sharing. 
%In both of the studies \cite{cortellessa2012enabling} and \cite{balsamo2004experimenting}, a kind of \textit{Architectural Description Language} named \textit{Emilia}, is used as the architecture model. \textit{Emilia} provides 

\begin{figure}[ht]
  \centering
  \includegraphics[width=\columnwidth]{figures/matrix.png}  
  \caption{Example of Probability Matrix~\cite{jalali2011new}}
  \label{fig:matrix}
\end{figure}

\begin{figure}[ht]
  \centering
  \includegraphics[width=\columnwidth]{figures/DTMC.png}  
  \caption{Example of Discrete Time Markov Chain (DTMC)~\cite{jalali2011new}}
  \label{fig:DTMC}
\end{figure}

\textbf{3) Model Transformation: } For obtaining the predicted performance metrics, the annotated meta-models have to be transformed to either performance engineering models, or simulation code that can be directly used as input of the simulation platforms. The transformation from the annotated architecture model to the performance engineering model as listed in the left three columns in Table~\ref{tbl:transformation}, e.g. \textit{Queuing Networks}, \textit{Stochastic Petri Nets}, and \textit{Stochastic Process Algebras}, is called \textit{Model-to-Model} transformation. The transformation from the annotated architecture model to the simulation code as listed in the right-most column in Table~\ref{tbl:transformation} is called \textit{Model-to-Text} transformation. 

In our reviewed studies, the \textit{Queuing Networks} are the most preferred performance models. As shown in Table~\ref{tbl:transformation}, in \textit{Model-to-Model} transformation studies, 60\% of the annotated architectural models are transformed into \textit{Queuing Networks}. A \textit{Queuing Network} model is a collection of interacting \textit{service centers} representing system resources, and a set of \textit{jobs} representing the users sharing the resources~\cite{pagliari2019extent, becker2008coupled}.  \textit{Jobs} travel through a network of \textit{service centers} using probabilistic routes. The analytical solution of \textit{Queuing Network} predicts the average response time of the overall system, waiting times for queues, average queue length, and server utilization~\cite{becker2008coupled}. A very simple example of \textit{Queuing Network} is illustrated as Figure~\ref{fig:queuing-network}. It depicts a closed workload scenario which has been mentioned above. A delay server models the ``think time'' which is indicated by the clock at the bottom. After a processing step on the CPU, jobs either use a hard-drive (HDD) with a probability of 30\% or a network resource (NET) with a probability of 70\%.

\begin{figure}[ht]
  \centering
  \includegraphics[width=\columnwidth]{figures/queuing-network.png}  
  \caption{Example of Queuing Network~\cite{becker2008coupled}}
  \label{fig:queuing-network}
\end{figure}

As shown in Table~\ref{tbl: perf-model}, a certain type of \textit{Queuing Networks}, namely \textit{Product Form Queuing Network (PFQN)}, can compute the predicted results precisely in very short time. However, the application of \textit{PFQN} is very restrictive because many realistic system, such as priority queues, is not in product form. From our observation, the \textit{PFQN} is only used to model ``Toy Projects'' that are rather simple and self-developed by developer, which we will describe in later section~\cite{jalali2011new, sharma2005architecture, zhang2010improving}. To model real-life, complicated software systems, several enhancements of \textit{Queueing Networks} exist, such as \textit{Layered Queuing Network (LQN)}~\cite{mani2011towards, arcelli2013software, di2004compositional, arcelli2015control, wu2015exploring, cortellessa2006software, das2004computing, martens2010automatically} and \textit{Extended Queuing Network (EQN)}~\cite{pooley2010cpasa, trubiani2011detection, eramo2012performance}. In \textit{LQN}, servers can issue requests to other servers during the processing of a job for their client. Software entities and hardware entities are represented as nodes in an acyclic graph. This acylic graph depicts the dependencies of node during job processing~\cite{mani2011towards, cortellessa2006software}. \textit{EQN} provides different colored highlighting spots that represents different control flow constructs like forks, branches, or backware jumps~\cite{pooley2010cpasa}. 

In Table~\ref{tbl:transformation}, in \textit{Model-to-Model} transformation studies, 30\% annotated architecture models were transformed into \textit{Stochastic Petri Net}. A \textit{Stochastic Petri Net} consists of a set of places and transitions, which are traversed by tokens~\cite{becker2008coupled, balsamo2004model}. Transitions remove and add tokens on places whenever they are active. \textit{Stochastic Petri Net} is well suited to analyze concurrent behavior and relevant properties such as deadlock freedom~\cite{xu2006evaluating, eismann2019integrating, becker2008coupled}. \textit{Generalized Stochastic Petri Net (GSPN)} is viewed as a formalism for the description of the global behavior of complex structures. It is the most basic form of \textit{Stochastic Petri Net}. \textit{GSPN} include two classes of transitions: 1) exponentially distributed timed transitions, which are used to model the random delays associated with the execution of activities; and 2) the immediate transitions, which represent the logical actions that do not consume time. Immediate transitions permits the existing of branching probabilities that are independent of timing specification~\cite{balbo2007introduction}. \textit{Colored Petri Net} provides a framework for the construction and analysis of distributed systems~\cite{xu2006evaluating}. It has the advantage of describing the behavior of the resource sharing and synchronization. \textit{Queuing Petri Net} is the combination of \textit{Queuing Network} and \textit{Colored Petri Net} that can easily model hardware contention and scheduling strategies as well as software contention, synchronization, blocking, and asynchronous processing~\cite{brosig2014quantitative}.

In Table~\ref{tbl:transformation}, in \textit{Model-to-Model} transformation studies, 10\% annotated architecture models were transformed into \textit{Stochastic Process Algebras}. The advantage of using \textit{Stochastic Process Algebras} is that they allow the integration of functional and nonfunctional aspects and provide a unique reference model for software specification and performance~\cite{balsamo2004model}. Three different sub-types of \textit{Stochastic Process Algebra} were used in the selected studies, e.g. \textit{Time Processes and Performability Evaluation (TIPP)}~\cite{pooley2010cpasa, balsamo2004model}, \textit{Extended Markovian Process Algebra (EMPA)}~\cite{kang2006performance}, and \textit{Performance Evaluation Process Algebra (PEPA)} ~\cite{balsamo2004experimenting}. All of them associate with exponentially distributed random variables to actions. Besides exponential actions, passive and immediate actions are also considered~\cite{balsamo2004model}. \textit{TIPP} is suitable for describing the behavior of a system because it is achieve by the convention that a certain random distribution function is associated with every action~\cite{hermanns1994performance}. In \textit{TIPP}, each action is represented as a pair consisting of an action name and the according random distribution function. \textit{EMPA} enhances the expressiveness of classical processes algebras in two ways. First, it offers actions whose duration is exponentially distributed as well as immediate actions, hence it is useful for performance abstraction. Second, the actions are able to be parameterized by priority levels and weights, hence the prioritized choices and probabilistic choices can be implemented~\cite{bernardo1996extended}. \textit{PEPA} also extends classical process algebras by introducing probabilistic branching and the timing of transitions, but it is more automated since it has been compacted into \textit{Eclipse} plugins. 

\begin{table*}
\setlength{\tabcolsep}{12pt}
\caption{Statistics of Model Transformation}
\begin{adjustbox}{width = 2\columnwidth,center}
\centering
\begin{tabular}{| l | c | c | c || c |} 
\hline
 \multirow{2}{*}{Architecture Model} & \multicolumn{3}{|c|}{Model-to-Model Transformation} & \multicolumn{1}{|c|}{Model-to-Text Transformation} \\ \cline{2-5}
 
 & Queuing Networks & Stochastic Petri Nets  & Stochastic Process Algebra  &  Simulation Code \\ \hline
 
 UML Diagrams & \cite{pooley2010cpasa, eramo2012performance, balsamo2004model, wu2015exploring, sharma2005architecture, balsamo2005performance, cortellessa2006software, trubiani2013model, mani2011towards, du2015evolutionary, arcelli2013software, di2004compositional, das2004computing, arcelli2019exploiting} & \cite{perez2010performance, das2004computing, balsamo2004model, moscato2007software, babar2004comparison, gokhale2006performance} & \cite{balsamo2004model} & \cite{de2008rup, li2016evaluating, balsamo2004model, park2006design, hauck2011ginpex, moreno2008performance, eskenazi2004analysis} \\ \hline
 
 Palladio Component Model & \cite{martens2010automatically, brosig2011automated, brosig2014quantitative} & \cite{brosig2014quantitative} & \cite{brosig2014quantitative} & \cite{martens2010automatically, kapova2010performance, noorshams2014enriching, brosig2011automated, kang2006performance, yasaweerasinghelage2018predicting, becker2013performance, brosig2014quantitative} \\ \hline
 
 Descartes Modeling Language & / & \cite{eismann2019integrating, eismann2018modeling} & / & / \\ \hline
 
 Architectural Description Language & / & \cite{xu2006evaluating} & \cite{balsamo2004experimenting} & \cite{cortellessa2012enabling, sharafi2010analytical} \\ \hline
 
 Probability Matrix & \cite{jalali2011new, zhang2010improving, sharma2005architecture} & / & / & / \\ \hline
\end{tabular}

\end{adjustbox}
\label{tbl:transformation}

\end{table*}


\begin{table*}[h!]
\small
\setlength{\tabcolsep}{12pt}
\caption{Output of Model Transformation}
\begin{center}
\begin{tabular}{ |c|c|c|c| } 
\hline
Perf Type & Description & Extension  & Reference \\
\hline
\multirow{3}{4em}{Queuing Networks} & \multirow{3}{23em}{A network of queues where user or transitions (represented as \textit{customers}) queue for system resources (represented as \textit{service centers}).} & Product Form Queuing Network  & \cite{jalali2011new, sharma2005architecture, zhang2010improving}   \\ \cline{3-4}
& &  Layered Queuing Network &  \cite{mani2011towards, arcelli2013software, di2004compositional, arcelli2015control, wu2015exploring, cortellessa2006software, das2004computing, martens2010automatically, pagliari2019extent, brosig2011automated, balsamo2004experimenting} \\ \cline{3-4}
& & Extended Queueing Network  & \cite{pooley2010cpasa, trubiani2011detection, eramo2012performance}  \\ \cline{1-4}
\multirow{3}{4em}{Stochastic Petri Nets} & \multirow{3}{23em}{A directed bipartite graph that consists of a set of \textit{places} (i.e. conditions, represented by circles) and \textit{transitions} (i.e. events that may occur, represented by bars).} & Queuing Petri Net & \cite{eismann2019integrating, brosig2014quantitative} \\ \cline{3-4}
&  & Colored Petri Net  & \cite{xu2006evaluating}  \\  \cline{3-4}
&  & Generalized Stochastic Petri Net  & \cite{gokhale2006performance, li2016evaluating, moscato2007software, perez2010performance} \\ \cline{1-4}
\multirow{3}{4em}{Stochastic Process Algebra} & \multirow{2}{23em}{Abstract languages used to describe sequential behaviors which may run concurrently, and synchronizations or communications between them.} & TIPP & \cite{balsamo2004experimenting} \\ \cline{3-4}
&  & EMPA  & \cite{balsamo2004model}  \\  \cline{3-4}
&  & PEPA  & \cite{brosig2014quantitative} \\ \hline\hline
\multirow{5}{4em}{Simulation Code} & \multirow{5}{23em}{The programming code generated from the instances of \textit{PCM} that can be directly used for the discrete-event simulation.} & SimuCom & \cite{martens2010automatically, kapova2010performance, brosig2011automated, yasaweerasinghelage2018predicting, balsamo2004model, brosig2014quantitative}\\ \cline{3-4}
& & PerOpteryx & \cite{trubiani2011detection, martens2010automatically} \\ \cline{3-4}
& & SimuLizar & \cite{becker2013performance} \\ \cline{3-4}
& & EventSim & \cite{wu2015exploring} \\ \cline{3-4}
& & GMPIF & \cite{eramo2012performance, eramo2012performance, li2016evaluating, de2008rup} \\ \cline{3-4}
\hline
\end{tabular}
\end{center}
\label{tbl: perf-model}
\end{table*}


\textbf{Model-to-Model Transformation: } This transformation transforms an instance of the source model, i.e. the annotated architecture model, into an instance of the target model. i.e. the performance engineering model, by using transformation rules~\cite{becker2008coupled}. In our study, the most frequently used transformation rule is graph-based transformation. Because all the top four rows in Table~\ref{tbl:transformation}, e.g. the \textit{UML Diagram}, the \textit{Palladio Component Model}, the \textit{Descartes Modeling Language}, and the \textit{Architectural Description Language}, can be defined as graphs. Graph-based transformation applies graph-grammars to models which are interpreted as graphs of objects. The graph-grammar consists of a source model pattern and a target model pattern. Whenever any left-hand side pattern matches to an object-sub-graph of the source model, that part of the source model is replaced by the structure given by the right-hand side pattern. This replacement process is repeated until all the patterns in the source model are transformed into the patterns in the target model~\cite{becker2008coupled}.

%A transformation rule consists of two parts: a left-hand side which accesses the source model, and the right-hand side which expands in the target model~\cite{czarnecki2003classification}. Both sides can be represented by any mixture of the following: 1) Variables, which hold elements from the source and target models; 2) Patterns, which are model fragments with a set of variables; and 3) Logic, which expresses computations and constraints on model elements~\cite{czarnecki2003classification}. In \textit{Model-to-Model} transformation, there is a wide range of types of transformation rules, such as direct manipulation, relational transformation, graph-based transformation, or hybrid approaches~\cite{becker2008coupled}. 

%In our study, the most frequently used transformation rule is graph-based transformation, since all the \textit{UML Diagram}, \textit{Palladio Component Model}, \textit{Descartes Modeling Language}, and the \textit{Architectural Description Language} are defined as graphs. 

As shown in Table~\ref{tbl:transformation}, 50\% of the annotated \textit{UML Diagrams} were transformed into \textit{Queuing Networks} by using the graph-based transformation~\cite{pooley2010cpasa, eramo2012performance, balsamo2004model, wu2015exploring, sharma2005architecture, balsamo2005performance, cortellessa2006software, trubiani2013model, mani2011towards, du2015evolutionary, arcelli2013software, di2004compositional, das2004computing, arcelli2019exploiting}. This process uses the transformation technique named \textit{XML Metadata Interchange (XMI)}, which maps the components in the \textit{UML Diagram} to services centers in the \textit{Queuing Network}, and the use case in the \textit{UML Diagram} to job classes in the \textit{Queuing Network}. 

%The advantage of the \textit{Model-to-Model} transformation is its flexibility. Because the annotated architecture models can be transformed into several possible performance models. 

As shown in Table~\ref{tbl:transformation}, 25\% of the \textit{UML Diagrams}, all of the \textit{Descartes Modeling Language}, and 50\% of the \textit{Architectural Description Language} were transformed into either \textit{Stochastic Petri Nets}~\cite{perez2010performance, das2004computing, balsamo2004model, moscato2007software, babar2004comparison, gokhale2006performance, eismann2019integrating, eismann2018modeling, xu2006evaluating} or \textit{Stochastic Process Algebra}~\cite{balsamo2004model, balsamo2004experimenting}. We categorize these transformations together because they have the commonality that used the intermediate model such as the \textit{Kernel Language for Performance and Reliability Analysis (KLAPER)}~\cite{becker2008coupled, becker2013performance, balsamo2004experimenting, gokhale2006performance, eismann2019integrating}. Similar to the graph-based transformation, \textit{KLAPER} is also based on the concept of components which offer services and the connectors that specify the behavior of these services. However, instead of transforming the patterns separately, the annotated architecture model is transformed into \textit{KLAPER} as a whole, then \textit{KLAPER} is transformed automatically into the performance engineering models. This significantly reduces the overall amount of transformations.

%An approach to deal with this transformation is the \textit{Kernel Language for Performance and Reliability Analysis (KLAPER)}~\cite{becker2008coupled, becker2013performance, balsamo2004experimenting, gokhale2006performance, eismann2019integrating}. \textit{KLAPER} is a meta-model designed to serve as the intermediate model for \textit{Model-to-Model} transformations. Similar to the graph-based transformation, e.g. \textit{XMI}, \textit{KLAPER} is also based on the concept of components which offer services and the connectors that specify the behavior of these services. However, instead of transforming the patterns separately, the annotated architecture model is transformed into \textit{KLAPER} as a whole, then \textit{KLAPER} is transformed automatically into the performance engineering models. This significantly reduces the overall amount of transformations.

As shown in Table~\ref{tbl:transformation}, 38\% of the \textit{Palladio Component Model} were transformed into performance engineering models. The \textit{Model-to-Model} transformation process for the \textit{Palladio Component Model} are different from that of the \textit{UML Diagrams}, \textit{Descartes Modeling Language}, and the \textit{Architectural Description Language}, because it is highly automated. In the default working platform of \textit{PCM}, \textit{Palladio Workbench}~\cite{yasaweerasinghelage2018predicting}, there exists the tools like \textit{PCM2LQN} and \textit{PCM2QPN}, which automatically transforms \textit{PCM} into \textit{Layered Queuing Network} and \textit{Queuing Petri Net}, respectively~\cite{brosig2014quantitative}. The core concept of these transformation tools is to firstly translate the created \textit{PCM} into \textit{XML}, then construct the performance models from the generated \textit{XML} file.

%This process of model transformation is based on the meta-model stored in the concrete syntax as defined by \textit{XML}. The technique of \textit{Model-to-Model} transformation for many architecture modeling languages, such as \textit{Palladio Component Model}, \textit{UML Diagrams}, and \textit{Architecture Description Language}, is \textit{XML Metadata Interchange (XMI)}, which can transform the meta-model in \textit{XML} format into a tree format, then map the nodes in the tree format into the elements in the performance engineering model~\cite{becker2008coupled}.
It is noticeable that since the \textit{Probability Matrix} is annotated by \textit{Markov Process} into a \textit{Discrete-Time Markov Chain (DTMC)}, which can be directly used as the input of \textit{Product Form Queuing Network}, the transformation process of such studies is neglected.




%map the concrete syntax into the elements in the performance engineering models~\cite{becker2008coupled}. 




\textbf{Model-to-Text Transformation: }This transformation can be regarded as a special class of \textit{Model-to-Model} transformation where the target model is simply a text file, i.e. simulation code in our study. 

%The advantage of \textit{Model-to-Text} transformation is the high automation of the process. However, its disadvantage is the time consumption for getting the sufficiently precise results, especially for large-scale, complex systems. 

As shown in Table~\ref{tbl: perf-model}, 75\% of the \textit{Palladio Component Models} that appeared in our reviewed studies applied \textit{Model-to-Text} transformation by using the existing techniques named \textit{PCM2SimuCom}~\cite{martens2010automatically, kapova2010performance, noorshams2014enriching, brosig2011automated, kang2006performance, yasaweerasinghelage2018predicting, becker2013performance, brosig2011automated, brosig2014quantitative}. \textit{PCM2SimuCom} has been compacted as an \textit{Eclipse} plugin. It can translate the instances of the annotated  \textit{Palladio Component Model} into executable Java code which can be loaded by the default simulation platform, the \textit{SimuCom}~\cite{yasaweerasinghelage2018predicting}. In the \textit{PCM} related studies, the process of translating instances into Java code are also applied by other automated simulation platform, such as \textit{SimuLizar}~\cite{becker2013performance} and \textit{PerOpteryx}~\cite{trubiani2011detection, martens2010automatically}. The difference of these simulation platforms will be explained later. 

%The \textit{Model-to-Text} transformation for \textit{Palladio Component Model} has existing techniques named \textit{PCM2SimuCom}~\cite{martens2010automatically, kapova2010performance, noorshams2014enriching, brosig2011automated, kang2006performance, yasaweerasinghelage2018predicting, becker2013performance, brosig2011automated, brosig2014quantitative}. 

The \textit{Model-to-Text} transformation for \textit{UML Diagrams} is also highly automated. As shown in Table~\ref{tbl:transformation}, 25\% of the \textbf{UML Diagrams} that appeared in our reviewed studies applied \textit{Model-to-Text} transformation. The \textit{Janus Transformation Language (JTL)} suites for the change propagation analyzing and translating for \textit{UML Sequence Diagram} and \textit{UML Use Case Diagram}~\cite{eramo2012performance, eramo2012performance, li2016evaluating, de2008rup}. The \textit{JTL} transformation has been also compacted into \textit{Eclipse} plugins~\cite{eramo2012performance}. By using \textit{JTL}, the \textit{UML Diagrams} are firstly translated into \textit{Generalized Performance Interchange Format (GMPIF)}, which is a good description of the information requirements for model interchange~\cite{smith2004performance}. 

%The \textit{Model-to-Text} transformation for \textit{Architectural Description Language}, \textit{Message Sequence Chart}, and \textit{Descartes Modeling Language} are not found in our selected studies. But it is noticeable that since the \textit{Probability Matrix} is annotated by \textit{Markov Process} into a \textit{Discrete-Time Markov Chain (DTMC)}, which can be directly used as the input of \textit{Product Form Queuing Network}, the transformation process of such studies is neglected.

\textbf{4) Model Solution: } Predicted performance metrics such as response time are obtained by solving the performance models. There are two different ways of solving the performance models: by simulation~\cite{martens2010automatically, noorshams2014enriching, brosig2011automated, balsamo2004experimenting, kang2006performance, yasaweerasinghelage2018predicting, becker2013performance, brosig2011automated, brosig2014quantitative, eskenazi2004analysis, park2006design, hauck2011ginpex, brosig2012modeling, groenda2012improving} and by analytical techniques~\cite{perez2010performance, das2004computing, balsamo2004experimenting, pagliari2019extent, jalali2011new, pooley2010cpasa, eramo2012performance, eismann2019integrating, xu2006evaluating, li2016evaluating, balsamo2004model, eismann2018modeling, sharafi2010analytical, di2004compositional, wu2015exploring, sharma2005architecture, moreno2008performance, balsamo2005performance, moscato2007software, trubiani2013model}. 

Simulation is an imitation of the operations of a system monitored over a period of time~\cite{pooley2010cpasa}. The advantage of simulation is the high degree of accuracy~\cite{becker2008coupled, pooley2010cpasa}. However, the disadvantage of simulation is that it is very time consuming, especially for large-scale complex systems~\cite{becker2008coupled, balsamo2004experimenting}. 6 out of 14 studies that used simulation applies \textit{SimuCom} as the simulation tool~\cite{martens2010automatically, kapova2010performance, brosig2011automated, yasaweerasinghelage2018predicting, balsamo2004model, brosig2014quantitative}. \textit{SimuCom} is the default simulator of \textit{PCM} and it is based on transformation of the \textit{PCM} instance to a process-based discrete-event simulation~\cite{brosig2014quantitative}. Another \textit{PCM} simulator, \textit{PerOpteryx}, that also takes instances of the annotated meta-model from \textit{PCM} as the input, has been compacted as a set of plugins embedded in \textit{Eclipse}~\cite{trubiani2011detection, martens2010automatically}. \textit{SimuLizar}, which was used in the study~\cite{becker2013performance}, is also an \textit{Eclipse} plugin that also takes \textit{PCM}'s meta-model as its input. \textit{SimuLizar} is a more comprehensive tool that not supports the simulation process to obtain the predicted performance metrics, but also supports the analysis for scalability, flexibility, and reliability. \textit{EventSim} is faster than \textit{SimuCom} and suites for systems with very high concurrency. In the study~\cite{wu2015exploring}, \textit{EventSim} was used to get the simulation results of a \textit{Layered Queuing Network} performance model and this study predicted the performance of a real-life open sourced project, \textit{Hadoop}. Some performance models have their specific simulation solvers. For example, \textit{LQN Simulation} is the default simulation solver for \textit{Layered Queuing Network}~\cite{eskenazi2004analysis, park2006design}, and \textit{SimQPN} is the the default simulation solver for \textit{Queing Petri Net}~\cite{brosig2014quantitative}.

Analytical solution only works for a range of performance models with very limited assumption, but solving analytically is much faster than simulation~\cite{pooley2010cpasa}. Usually, the performance models have default analytical solution tool. \textit{Symbolic Hierarchical Automated Reliability and Performance Evaluator (SHARPE)} is a very useful analytical solution tool that contains algorithms for the analysis of fault trees, acyclic series-parallel graphs, and Markov or semi-Markov models~\cite{trivedi2002sharpe}. In our selected studies, all the studies that use \textit{Product Form Queuing Network} which are produced from \textit{Discrete Time Markov Chain} use \textit{SHARPE} to provide analytical solution~\cite{jalali2011new, sharma2005architecture, zhang2010improving}. The \textit{Layered Queuing Network} has its default analytical solver named \textit{LQN Solver (LQNS)}, which provides fast numeric approximation for \textit{LQN} models~\cite{ani2011towards, di2004compositional, wu2015exploring, cortellessa2006software, martens2010automatically, pagliari2019extent, balsamo2004experimenting}. Similarly, \textit{Queuing Petri Net} has its default solver named \textit{QPN Solver}~\cite{eismann2019integrating}. \textit{GreatSPN} is a graphical user interface written in \textit{Java} language that can be used to draw \textit{Generalized Stochastic Petri Nets (GSPN)}~\cite{li2016evaluating, balsamo2004model}. It is a highly automated tool that has a rich set of graphical elements representing immediate and exponential transitions of \textit{GSPN}. The analytical solution of \textit{Stochastic Algebra Process} usually uses an efficient algorithm for state space generate to transform the algebra into a semi-Markov process~\cite{balsamo2005performance}. This approach has been implemented using the tool \textit{DSPNexpress 2000}~\cite{lindemann2000quantitative}, which supports the quantitative analysis of discrete-even stochastic processes. After that, the generalized semi-Markov model can be solved by using tools such as \textit{SHARPE}, etc. 

==> rq2.tex <==
\subsection{RQ-2: Development Activities}
\label{sec:rq2}

\begin{comment}

\begin{table*}[h]
%\setlength\extrarowheight{2pt}
\setlength{\tabcolsep}{8pt}
\centering
\caption{Proportion of Study Purposes with Facilitated Development Activity}\label{Tab1}
\begin{tabular}{@{}lccccc}   
\hline
\textbf{Development Activity} &  \textbf{Design} & \textbf{Implementation} & \textbf{Deployment} & \textbf{Operation} & \textbf{Maintenance} \\[0.75ex] \hline\hline
1. Model-based Performance Analysis & \cellcolor[HTML]{656565}\color[HTML]{FFFFFF} 48 (70\%) & 4 (6\%) & 1 (1\%) & 8 (12\%) & 9 (13\%) \\ 
\indent{} 1.1. Performance Prediction & \cellcolor[HTML]{656565}\color[HTML]{FFFFFF} 45 (74\%) & 4 (7\%) & 1 (2\%) & 8 (13\%) & 6 (10\%) \\
\indent{} 1.2 Root Cause Analysis & 0 & 0 & 0 & 0 & \cellcolor[HTML]{656565}\color[HTML]{FFFFFF} 3 (100\%) \\
\indent{} 1.3 Architectural Optimization & \cellcolor[HTML]{656565}\color[HTML]{FFFFFF} 3 (100\%) & 0 & 0 & 0 &  0  \\ \hline
2. Performance Anti-patterns Detection and Solution & \cellcolor[HTML]{656565}\color[HTML]{FFFFFF} 10 (67\%) & 0 & 0 & 0 & 5 (33\%) \\ \hline
3. Profiling and Comparison & \cellcolor[HTML]{656565}\color[HTML]{FFFFFF} 4 (67\%) & 0 & 2 (33\%) & 0 & 0 \\ \hline
4. Self-Adaption & 1 (17\%) & 0 & 1 (17\%) & \cellcolor[HTML]{656565}\color[HTML]{FFFFFF} 5 (83\%) & 0 \\ \hline\hline

\textit{All} & \cellcolor[HTML]{656565}\color[HTML]{FFFFFF} 65 (69\%) & 5 (5\%) & 4 (4\%) & 13 (14\%) & 14 (15\%) \\ \hline
\end{tabular}
\label{tbl:life-cycle}
\end{table*}

\end{comment}

\begin{table*}[h]
%\setlength\extrarowheight{2pt}
\setlength{\tabcolsep}{8pt}
\centering
\caption{Proportion of Study Objectives according to Life-cycle Phase}\label{Tab1}
\begin{tabular}{@{}lccccc}   
\hline
\textbf{Development Activity} &  \textbf{Design} & \textbf{Implementation} & \textbf{Deployment} & \textbf{Operation} & \textbf{Maintenance} \\[0.75ex] \hline\hline
1. Model-based Performance Analysis & \cellcolor[HTML]{656565}\color[HTML]{FFFFFF} 50 (48\%) & 4 (4\%) & 1 (1\%) & 8 (8\%) & 9 (9\%) \\ 
\indent{} 1.1. Performance Prediction & \cellcolor[HTML]{656565}\color[HTML]{FFFFFF} 46 (44\%) & 4 (4\%) & 1 (1\%) & 8 (8\%) & 6 (6\%) \\
\indent{} 1.2 Retrospective Root Cause Analysis & 0 &  0 & 0 & 0 & \cellcolor[HTML]{656565}\color[HTML]{FFFFFF} 4 (4\%) \\
\indent{} 1.3 Architectural Optimization & \cellcolor[HTML]{656565}\color[HTML]{FFFFFF} 3 (3\%) & 0 & 0 & 0 &  0  \\ \hline
2. Performance Anti-patterns Detection and Solution & \cellcolor[HTML]{656565}\color[HTML]{FFFFFF} 10 (10\%) & 1 (1\%) & 1 (1\%) & 0 & 5 (5\%) \\ \hline
3. Profiling and Comparison &  \cellcolor[HTML]{656565}\color[HTML]{FFFFFF} 4 (4\%) & 0 & \cellcolor[HTML]{656565}\color[HTML]{FFFFFF} 4 (4\%) & 2 (2\%) & 1 (1\%) \\ \hline
4. Self-Adaption & 1 (1\%) & 0 & 2 (2\%) & \cellcolor[HTML]{656565}\color[HTML]{FFFFFF} 6 (6\%) & 0 \\ \hline\hline

\textit{All} & \cellcolor[HTML]{656565}\color[HTML]{FFFFFF} 67 (64\%) & 6 (6\%) & 8 (8\%) & 16 (15\%) & 15 (14\%) \\ \hline
\end{tabular}
\label{tbl:life-cycle}
\end{table*}


RQ2 analyzes the development activities that different studies aimed to facilitate, and maps the identified activities to the research objectives from RQ1. This provides guidance for practitioners to identify the most relevant techniques for the development activities they are engaged in.

Five software development activities (or phases) emerged from our analysis: 1) \textit{Software Design} when the developers focus on the high-level and preliminary architecture and design of their systems; 2) \textit{Software Implementation} when developers implement and test their systems; 3) \textit{Software Deployment} when developers launch their systems in the physical environment; 4) \textit{Software Operation} when developers focus on the run-time behavior of their systems in the product environment; and 5) \textit{Software Maintenance} when developers keep updating and supporting existing systems to solve arising issues. 


In Table~\ref{tbl:life-cycle},  rows 2 to 5 show the number and percentage of studies in each purpose that addressed each development phase. The cells colored grey highlight the largest numbers in each  category. The bottom row in Table~\ref{tbl:life-cycle}, (``\textit{All}''), shows the total number (and percentage) of studies for each phase. Next we  elaborate the details of each study purpose.

\subsubsection{\textbf{Purpose 1: Model-based Performance Analysis:}} 

%\textcolor{blue}{Most (70\%) of the studies in \textit{Purpose-1} facilitate software design~\citeS{mani2013propagation,kapova2010performance,hauck2011ginpex,litoiu2013performance,happe2014stateful,geetha2011framework,wrzosk2012applying,becker2013performance,tribastone2010performance,barbierato2012perfbpel,eshraghian2015performance,gomez2014performance,jalali2011new,wu2015exploring,smith2017spe,werle2020data,requeno2017performance,nalepa2015model,berardinelli2010performance,kross2017model,yasaweerasinghelage2018predicting,noorshams2014enriching,maddodi2020aggregate,pinciroli2020model,gribaudo2018performance,nguyen2017parad,gaudel2011ada,woodside2014transformation,happe2010parametric,trubiani2013model,etxeberria2014performance,tawhid2011automatic,brosig2014quantitative,groenda2012improving,kapova2010systematic,gorsler2014performance,eismann2019integrating,naddaf2013performance,hauck2010automatic,gomez2018enabling,arcelli2013software,trubiani2015exploiting,alhaj2013traceability,eramo2012performance,trubiani2020visarch,koziolek2011peropteryx,du2015evolutionary,martens2011monolithic}. Besides that, the studies in \textit{Purpose-1} can also facilitate the other four development activities, including implementation (6\%)~\citeS{kapova2010performance, hauck2011ginpex, mazkatli2020incremental}, deployment (1\%)~\citeS{khan2010performance}, operation (12\%)~\citeS{ mazkatli2020incremental,arcelli2015control,hill2010run,von2011performance,brosig2014architecture,eismann2018modeling,huber2016model,arcelli2019exploiting}, and maintenance (13\%)~\citeS{brosig2011automated,gambi2010model,krogmann2010using,walter2017expandable,brunnert2017continuous,li2016evaluating,wu2020microrca,zhao2020butterfly,zhao2020performance}.}

%\textcolor{blue}{In general, most (70\%) of the studies in \textit{Purpose-1} facilitate software design. Besides that, the studies in \textit{Purpose-1} may also facilitate the other four development activities, including implementation (6\%), deployment (1\%), operation (12\%), and maintenance (13\%).}
%We found that the three sub-categories---1.1 performance prediction, 1.2 Root Cause Analysis, and 1.3 Architectural Optimization, had the respective development activities that they mainly focused on.

In \textit{Category-1.1 Performance Prediction}, most studies  (\textcolor{red}{70\%}) 
aimed at facilitating software design ~\citeS{happe2014stateful,wrzosk2012applying,gomez2014performance,barbierato2012perfbpel,becker2013performance,tribastone2010performance,geetha2011framework,eshraghian2015performance,jalali2011new,smith2017spe,requeno2017performance,kross2017model,wu2015exploring,gribaudo2018performance,maddodi2020aggregate,werle2020data,noorshams2014enriching,yasaweerasinghelage2018predicting,nalepa2015model,berardinelli2010performance,nguyen2017parad,gaudel2011ada,brosig2014quantitative,eismann2019integrating,gomez2018enabling,woodside2014transformation,happe2010parametric,hauck2010automatic,groenda2012improving,kapova2010systematic,tawhid2011automatic,naddaf2013performance,trubiani2013model,etxeberria2014performance,gorsler2014performance,trubiani2020visarch,eramo2012performance,alhaj2013traceability,arcelli2013software,trubiani2015exploiting,kwon2013mantis,kapova2010performance,hauck2011ginpex,litoiu2013performance, pinciroli2021model, klinaku2021architecture}. These studies conducted  early performance assessments based on  design models. The performance metrics predicted based on these models helps to evaluate early design choices, to avoid  rework before a system is implemented. 
Four studies (7\%) in category-1.1 focused on software implementation~\citeS{kapova2010performance, hauck2011ginpex, mazkatli2020incremental, mani2013propagation}. These approaches  automatically detect  source code changes and reflect such changes in software models. With these updated models developers could quickly evaluate the impact of code changes on performance. Only one study aimed at software deployment~\citeS{khan2010performance}. It investigated the optimal deployment mapping of software components onto hardware devices. 
Eight (13\%) studies targeted run-time performance prediction~\citeS{litoiu2013performance,mazkatli2020incremental,arcelli2015control,brosig2014architecture,hill2010run,eismann2018modeling,huber2016model,von2011performance}. They calibrated performance models with resource usage profiles while systems were running. Six (10\%) studies targeted software maintenance~\citeS{brosig2011automated,krogmann2010using,walter2017expandable,gambi2010model,brunnert2017continuous,li2016evaluating}. They derived software models from existing systems and provided performance evaluation considering architectural evolution. 
%\lu{make sure the numbers in the description are consistent with Table~\ref{Tab1}}


%All four studies~\citeS{wu2020microrca,zhao2020butterfly,zhao2020performance, heger2013automated} in \textit{Category-1.2 Retrospective Root Cause Analysis} targeted  software maintenance. They all provided root cause analysis of performance issues in existing systems to provide guidance for developers during maintenance.

\textcolor{blue}{The four studies in Category-1.2 Retrospective Root Cause Analysis~\citeS{wu2020microrca, zhao2020butterfly, zhao2020performance, heger2013automated}  target the software maintenance phase. They perform a root cause analysis of performance issues in existing systems, providing  guidance for developers doing maintenance. For instance, Heger et al.~\citeS{heger2013automated}  aim to support software development by enabling engineers to distinguish between minor and major performance regressions for subsequent problem diagnosis. This approach allows developers to focus their optimization efforts on the most impactful performance regressions. The emphasis on software maintenance in these studies is because root cause analysis predominantly aids in identifying and rectifying performance issues in pre-existing systems. It is during the maintenance phase that such issues become apparent and must be addressed to ensure the system's ongoing performance and reliability.}

All three studies in \textit{Category-1.3 Model-based Architectural Optimization} aimed at facilitating better software design solutions~\citeS{arcelli2019exploiting,koziolek2011peropteryx,du2015evolutionary}. They 
provided support for stakeholders in performing architectural refactoring on design models.


\subsubsection{\textbf{Purpose 2: Performance Anti-pattern Detection and Resolution}} 

The majority of the studies in \textit{Purpose-2} (ten out of sixteen, or 63\%)~\citeS{cortellessa2010digging,cortellessa2014approach,trubiani2011detection,trubiani2014guilt,de2017model,arcelli2012antipattern,arcelli2018performance,arcelli2015performance,trubiani2014exploring,arcelli2017applying} focus on the identification and refactoring of performance anti-patterns during the software design phase. These studies  employ UML diagrams and \textit{PCM} as their analytical tools.

Conversely, five studies (31\%)~\citeS{fioravanti2017engineering, chen2014detecting, wert2013supporting, trubiani2018exploiting, wert2014automatic} emphasize the maintenance phase of software development. They apply dynamic profiling to existing software applications and use performance metrics to identify and eliminate anti-patterns, thus helping maintain the health and efficiency of the systems.

\textcolor{blue}{Additionally,  paper~\citeS{avritzer2021multivariate} extends this scope to include the implementation and deployment phases. This study introduces a novel approach for Software Performance Anti-pattern (SPA) characterization and detection,  designed to bolster continuous integration/delivery/deployment (CI/CDD) pipelines. This inclusion addresses the computational efficiency gaps in current detection algorithms,  enhancing performance across all development stages.}


\subsubsection{\textbf{Purpose 3: Profiling and Comparison}} 

%Out of the eleven studies in this category, four (36\%) focus primarily on the software design phase. These studies provide empirical insights regarding design choices, such as databases~\citeS{haughian2016benchmarking, fioravanti2016experimental}, web frameworks~\citeS{sunardi2019mvc}, and programming paradigms~\citeS{lung2014measuring}. Another three studies (27\%) emphasize the software deployment phase~\citeS{zulkipli2013empirical, avritzer2018quantitative, alzboon2022performance}. These papers offer a quantitative assessment and comparison of architecture alternatives for deployment with micro-services~\citeS{avritzer2018quantitative} and web-services~\citeS{zulkipli2013empirical}. They also discuss how their approaches can aid practitioners in making informed deployment decisions~\citeS{alzboon2022performance}.

\textcolor{blue}{In this category, four (36\%) studies,  \citeS{haughian2016benchmarking, fioravanti2016experimental, sunardi2019mvc, lung2014measuring}, concentrated on the software design phase by providing empirical experience regarding design choices like databases, web frameworks, and programming paradigms. Focusing on the  deployment phase, four (36\%) studies, \citeS{zulkipli2013empirical, avritzer2018quantitative, alzboon2022performance, avritzer2020scalability}, offer quantitative assessment and guidance for deployment decisions, including architectural comparisons and performance assessment of  deployment configurations in micro-services and web-services environments. Two (18\%) studies, \citeS{ngo2022evaluating, blinowski2022monolithic}, emphasized the operation phase by exploring the effectiveness of workload smoother  patterns and comparing the performance and scalability of different architectural styles in operational conditions. One study, \citeS{gonccalves2021monolith}, with a  focus on the maintenance phase, presented a detailed refactoring process, from a large monolithic to a modular system, analyzing the performance impact and refactoring effort.}


%Four (67\%) studies  in this category focused on software design as they provided empirical experience regarding design choices, such as databases~\citeS{haughian2016benchmarking, fioravanti2016experimental}, web frameworks~\citeS{sunardi2019mvc}, and programming paradigm~\citeS{lung2014measuring}. 

%The other two (33\%) studies in this category aimed at facilitating software deployment~\citeS{zulkipli2013empirical, avritzer2018quantitative}. They provided quantitative assessment and comparison of architecture alternatives for deployment with micro-services~\citeS{avritzer2018quantitative} and web-services~\citeS{zulkipli2013empirical}. 

%One study~\citeS{lung2014measuring} facilitates software development. It measures the impact of \textit{Aspect-oriented Programming (AOP)} that deals with scattered and tangled coding on system performance, and the experimental results show that \textit{AOP} does not have significant effect on software performance. Therefore, \citeS{lung2014measuring} encourages practitioners to apply \textit{AOP} during implementation, because \textit{AOP} improves the readability of source code. \lu{the choice of AOP is also a design choice, and should be for design. Please update table and writing.} 








\subsubsection{\textbf{Purpose 4: Self-Adaption}} 
Self-adaptive systems dynamically adjust their configuration at run-time to meet performance goals in changing environments. \textcolor{blue}{The majority of studies (77\%) focused on system operation at run-time~\citeS{lung2016improving, camara2020quantitative, camara2013evolving, gergin2014decentralized, arcelli2020multi, ezzeddine2021design}. Notably, two studies, \citeS{gergin2014decentralized} and \citeS{peng2021parallel}, went a step further and not only reconfigured the software components but also re-deployed resources in the deployment environment. Consequently, these studies also offer valuable insights for the deployment phase.} One study~\citeS{perez2010performance} focused on providing guidance for designing a self-adaptive system.


%Among them, \citeS{gergin2014decentralized} not only re-configured the software components, but also re-configured the physical resources allocation in the deployment environment. Thus, we considered this study as facilitating deployment as well.

%Most (83\%) of these studies addressed performance during system operation at run-time~\citeS{lung2016improving, camara2020quantitative, camara2013evolving, gergin2014decentralized, arcelli2020multi}. Among them, \citeS{gergin2014decentralized} not only re-configured the software components, but also re-configured the physical resources allocation in the deployment environment. Thus, we considered this study as facilitating deployment as well. One study~\citeS{perez2010performance} focused on providing guidance for designing a self-adaptive system.

\textbf{RQ2 Summary:} The techniques or methodologies from the 104 studies tackle challenges covering the five major phases of the software development life-cycle, namely \textit{Design}, \textit{Implementation}, \textit{Deployment}, \textit{Operation}, and \textit{Maintenance}. Overall, \textit{Design} is the most extensively covered. Table~\ref{tbl:life-cycle} provides a mapping between the four major categories of studies (from RQ1) onto the life-cycle phases. Readers can refer to this table to identify prior work that best matches their needs. It also sheds light on gaps are for future research. 


==> rq5-aspects.tex <==
\subsubsection{\textbf{Evaluation Purpose}} 


%\textcolor{blue}{28 (30\%) out of the 94 studies in our literature only assess the feasibility of the their proposed approaches~\citeS{arcelli2015control,barbierato2012perfbpel,arcelli2017applying,gambi2010model,groenda2012improving,eramo2012performance,arcelli2012antipattern,hill2010run,arcelli2020multi,geetha2011framework,litoiu2013performance,gribaudo2018performance,berardinelli2010performance,trubiani2013model,etxeberria2014performance,smith2017spe,trubiani2015exploiting,kapova2010systematic,tribastone2010performance,tawhid2011automatic,trubiani2014exploring,naddaf2013performance,gomez2018enabling,gaudel2011ada,woodside2014transformation,cortellessa2014approach,trubiani2018exploiting,trubiani2014guilt}. 
We discuss the evaluation aspects based on studies with different purposes.


\textbf{a) Evaluation of the \textit{Model-based Performance Analysis} studies:}
For Category-1.1 Performance Prediction (\textcolor{blue}{total 63 papers}), \textcolor{blue}{26 (40\%)} studies only conduct a case study to show the feasibility of the proposed approach, without providing any specific evaluation criteria~\citeS{barbierato2012perfbpel,geetha2011framework,litoiu2013performance,gribaudo2018performance,berardinelli2010performance,groenda2012improving,gambi2010model,etxeberria2014performance,trubiani2013model,eramo2012performance,arcelli2015control,hill2010run,khan2010performance,becker2013performance,kapova2010performance,smith2017spe,trubiani2015exploiting,tribastone2010performance,gaudel2011ada,kapova2010systematic,tawhid2011automatic,naddaf2013performance,gomez2018enabling,woodside2014transformation,nguyen2017parad, klinaku2021architecture}. In the other 25 (40\%) studies, researchers report the \textbf{prediction accuracy} of their approaches~\citeS{mazkatli2020incremental, martens2011monolithic,happe2014stateful,krogmann2010using,huber2016model,nalepa2015model,kwon2013mantis,brosig2011automated,li2016evaluating,brunnert2017continuous,noorshams2014enriching,hauck2010automatic,hauck2011ginpex,maddodi2020aggregate,eismann2018modeling,brosig2014quantitative,eismann2019integrating,walter2017expandable,happe2010parametric,requeno2017performance,werle2020data,yasaweerasinghelage2018predicting,brosig2014architecture,wu2015exploring,kross2017model}. For example, the prediction accuracy ranges from 90\% to 95\% in~\citeS{brosig2011automated, yasaweerasinghelage2018predicting, eismann2018modeling} when comparing to the actual performance metrics of the systems. In addition, six (10\%) studies also evaluate the \textbf{prediction efficiency}---i.e., the speed of their proposed prediction approaches~\citeS{huber2016model, von2011performance, brosig2014quantitative, eismann2019integrating, wrzosk2012applying, eshraghian2015performance}. For example, \citeS{eismann2019integrating} speeds up the prediction process by up to 94.8\% by comparing to a baseline prediction approach. In three (5\%) studies, researchers examine the \textbf{performance improvement} of the system after making performance optimization based on prediction results~\citeS{mani2013propagation, jalali2011new, gomez2014performance}. For example, \citeS{jalali2011new} reports ``\textit{18\% increase in throughput and 60\% decrease in average response time}'' after architectural refactoring based on the prediction results. Finally, three (5\%) studies evaluate the \textbf{manual effort} for practitioners when using the prediction approach~\citeS{martens2011monolithic, arcelli2013software, gorsler2014performance}. For example, \citeS{martens2011monolithic} reports the learning curve for 47  students using different prediction approaches based on questionnaires and screen recordings.

%In 27 (40\%) out of the 67 studies in \textit{Purpose-1}~\citeS{mazkatli2020incremental,happe2014stateful,krogmann2010using,huber2016model,nalepa2015model,kwon2013mantis,brosig2011automated,li2016evaluating,brunnert2017continuous,noorshams2014enriching,hauck2010automatic,hauck2011ginpex,maddodi2020aggregate,eismann2018modeling,brosig2014quantitative,eismann2019integrating,walter2017expandable,happe2010parametric,requeno2017performance,werle2020data,yasaweerasinghelage2018predicting,brosig2014architecture,wu2015exploring,kross2017model,zhao2020butterfly,wu2020microrca,martens2011monolithic}, researchers reported the \textbf{prediction accuracy} of their approaches. For example, the prediction accuracy ranges from 90\% to 95\% in~\citeS{brosig2011automated, yasaweerasinghelage2018predicting, eismann2018modeling}.
%In addition, 5 (8\%) studies in Category-1.1~\citeS{huber2016model, von2011performance, brosig2014quantitative, eismann2019integrating, wrzosk2012applying} also evaluate the \textbf{efficiency} (i.e., prediction speed) of their approaches. For example, in \citeS{eismann2019integrating}, its proposed approach ``\textit{maintains sufficient prediction accuracy and achieves speeds-up of up to 94.8\%}''. 
%Furthermore, 5 (7\%) studies~\citeS{mani2013propagation, jalali2011new, gomez2014performance} that provide architectural refactoring solutions examined the \textbf{performance improvement} of the system after refactoring. For example, in \citeS{arcelli2019exploiting}, the response time of the evaluated web-based system improved by 13.34\%. }

\textcolor{blue}{In category 1.2,  \textit{Retrospective Root Cause Analysis}, three studies focus on evaluating the \textbf{accuracy} and \textbf{effectiveness} of identifying performance bottlenecks~\citeS{zhao2020butterfly, wu2020microrca, heger2013automated}.} For instance, Zhao et al.~\citeS{zhao2020butterfly} report that their proposed \textit{Butterfly Space Modeling} method attains a 60\% recall rate in detecting methods with performance problems, compared to a 33\% recall rate when using traditional profiling techniques. Similarly, Wu et al.~\citeS{wu2020microrca} develop a technique known as \textit{MicroRCA}, which achieves an impressive 89\% precision rate in pinpointing the root causes of performance issues in micro-services. \textcolor{blue}{Moreover, Heger et al.~\citeS{heger2013automated} evaluate the \textit{effectiveness} of their approach. When a regression is detected, their system,  PRCA, automatically provides information about the change that caused the regression and the methods involved, offering a valuable tool for identifying and resolving performance issues.} In addition to accuracy and effectiveness, another study by Zhao et al.~\citeS{zhao2020performance} delves into the \textbf{Return on Investment (ROI)} of fixing various types of performance issues. Here, the 'investment' is quantified by the number of discussions and developers, and the 'return' is measured by the performance improvement observed after code revisions.

%In category-1.2, \textit{Retrospective Root Cause Analysis}, two studies evaluate the \textbf{accuracy} of identifying the performance bottlenecks~\citeS{zhao2020butterfly, wu2020microrca}. For example, \citeS{zhao2020butterfly} reports that the recall of detecting methods with performance problems by using the proposed \textit{Butterfly Space Modeling} is 60\%, compared to 33\% using profiling techniques. In \citeS{wu2020microrca}, the proposed approach, \textit{MicroRCA}, achieves 89\% precision in detecting root causes of performance problems in micro-services. The other study~\citeS{zhao2020performance} investigates the \textbf{Return on Investment (ROT)} of fixing different types of performance issues, where the investment is measured by the number of discussions and developers, and the return is measured by the performance improvement after code revisions.


In category-1.3 \textit{Model-based Architectural Optimization}, all three studies~\citeS{du2015evolutionary, koziolek2011peropteryx, arcelli2019exploiting} evaluate the \textbf{performance improvement} after applying alternative architectural solution for optimization. For example, in \citeS{arcelli2019exploiting}, the response time of the evaluated web-based system improves by 13.34\% after architectural refactoring.



%However, only 2 (4\%) studies in \textit{Purpose-1} have compared the prediction accuracy of their approaches with previous approaches~\citeS{li2016evaluating, du2015evolutionary}. This indicates the lack of a baseline for evaluating the \textit{Model-based Prediction} approaches. 

%\textbf{a) Evaluation of the \textit{Model-based Prediction} studies:} The effectiveness of the \textit{Model-based Prediction} approaches measures the \textbf{accuracy of the prediction}---the difference between the predicted and the actual performance metrics. Researchers sometimes also evaluate the \textbf{extent of performance improvement} after fixing the predicted performance problems. In \textcolor{black}{14 out of 53 (26\%)} studies in \textit{Purpose-1}, researchers reported prediction accuracy~\citeS{li2016evaluating, eismann2018modeling, eismann2019integrating, groenda2012improving, walter2017expandable,rak2017performance,noorshams2014enriching, yasaweerasinghelage2018predicting, brosig2011automated, happe2010parametric,kross2017model, martens2011monolithic, mazkatli2020incremental, huber2016model}. For example, the prediction accuracy ranges from 90\% to 95\% in~\citeS{brosig2011automated, yasaweerasinghelage2018predicting, eismann2018modeling}. 

%In addition, \textcolor{black}{some of the \textit{Model-based Prediction} studies provide an interpretation of the predicted results or the suggestion on architectural refactoring for performance improvement~\citeS{hauck2011ginpex, brosig2014architecture, spinner2016reference}.} Besides effectiveness, researchers also examine the performance and comprehensiveness of the predicted metrics by the proposed approaches. In 12\% of the \textit{Model-based Prediction} studies, researchers compared the performance of their approaches with existing techniques. For example, in~\citeS{eismann2019integrating}, researchers reported 94.8\% speedup while maintaining sufficient prediction accuracy by optimizing the solver using machine learning models.

%Researchers also evaluated the comprehensiveness of the predicted metrics~\citeS{kapova2010performance, brebner2012experiences}. One study~\citeS{kapova2010performance} revealed that most prediction focuses on three performance metrics---response time, resource utilization, and throughput. This is consistent with our finding --- 79\% of the \textit{Model-based Prediction} studies focus on all three metrics. In addition, in several studies~\citeS{wu2015exploring, li2016evaluating}, the proposed approaches can predict the best, worse, and the average of these three metrics. 

%(1) Effectiveness: Automated incremental transformations are explored and evaluated for effectiveness on a case study example; (2) Performance Improvement of Evaluation System: compare the RT and TP of with and without facade design pattern


\textbf{b) Evaluation of \textit{Performance Anti-pattern Detection and Solution} studies:}  studies presents various dimensions of focus. Five out of 16 (31\%) studies performed case studies to demonstrate the feasibility of their proposed methodologies, without implementing any distinct evaluation criteria~\citeS{arcelli2017applying, arcelli2012antipattern, trubiani2014exploring, trubiani2018exploiting, avritzer2021multivariate}.

Six (38\%) of these studies concentrated on the \textbf{accuracy} of anti-pattern detection~\citeS{arcelli2018performance, arcelli2015performance, wert2014automatic, wert2013supporting, de2017model, avritzer2021multivariate}. As an example, Wert et al.~\citeS{wert2014automatic} achieved an impressive 100\% precision and recall in detecting six distinct types of performance anti-patterns, including \textit{Blob / God Class}, \textit{Pipe and Filter}, \textit{Extensive Processing}, \textit{Traffic Jam}, \textit{One-Lane Bridge}, and \textit{Empty Semi Trucks}.

In total, eight (50\%) studies evaluated the extent of \textbf{performance improvement} resulting from the removal of performance anti-patterns~\citeS{de2017model, trubiani2011detection, cortellessa2010digging, chen2014detecting, wert2013supporting, trubiani2014guilt, fioravanti2017engineering, arcelli2018performance}. For instance, Trubiani et al.~\citeS{trubiani2014guilt} reported a performance improvement of 37\% to 84\% after eradicating the identified performance anti-patterns.

\textcolor{blue}{Finally, three (19\%) studies examined the \textbf{detection efficiency}—in other words, the speed of detecting performance anti-patterns~\citeS{cortellessa2014approach, de2017model, avritzer2021multivariate}. For example, the execution of the anti-pattern detecting approach proposed in \citeS{de2017model}  took just a few seconds.}

%Evaluation of \textit{Performance Anti-pattern Detection and Solution} studies:} 
%\textcolor{blue}{Four (25\%) of the 16 papers} only conducted case studies to show the feasibility of the proposed approach, without checking any evaluation criteria~\citeS{arcelli2017applying,arcelli2012antipattern,trubiani2014exploring,trubiani2018exploiting}. Five (34\%) studies focused on the \textbf{accuracy} of anti-pattern detection~\citeS{arcelli2018performance, arcelli2015performance, wert2014automatic, wert2013supporting, de2017model}. For example, in \citeS{wert2014automatic}, the precision and recall reached up to 100\% in detecting six types of performance anti-patterns, including \textit{Blob / God Class}, \textit{Pipe and Filter}, \textit{Extensive Processing}, \textit{Traffic Jam}, \textit{One-Lane Bridge}, and \textit{Empty Semi Trucks}.
%In eight (53\%) studies, researchers evaluated the extent of \textbf{performance improvement} resulting from eliminating the performance anti-patterns~\citeS{de2017model,trubiani2011detection,cortellessa2010digging,chen2014detecting,wert2013supporting,trubiani2014guilt,fioravanti2017engineering,arcelli2018performance}. For example, in \citeS{trubiani2014guilt}, after removing  performance anti-patterns,  system  performance improved from 37\% to 84\%. Finally, two (13\%) studies~\citeS{cortellessa2014approach, de2017model} examined the \textbf{detection efficiency}---i.e., the speed of detecting performance anti-patterns. For example, the execution of the anti-pattern detecting approach proposed in \citeS{de2017model} just took a few seconds.

\textbf{c) Evaluation of the \textit{Profiling and Comparison} studies:} \textcolor{blue}{The 11 studies here aimed to evaluate how architectural variables impact the performance of a software system. Some studies utilized controlled \textbf{workload} parameters, for instance, testing with varying numbers of simultaneous users~\citeS{sunardi2019mvc} and assessing resource usage under increased workload~\citeS{ngo2022evaluating}. Other studies compared systems under different \textbf{use case scenarios} such as benchmarking databases under heavy-read and heavy-write conditions~\citeS{haughian2016benchmarking}, and comparing the stability of distinct blogging systems~\citeS{alzboon2022performance}. The \textbf{impact of hardware resources} was another aspect investigated, as demonstrated by studies examining the influence of CPU cores on deployment performance~\citeS{avritzer2018quantitative} and system scalability under varied workloads~\citeS{avritzer2020scalability}. Further evaluations considered the role of number of machines, programming language, and scaling on system performance~\citeS{blinowski2022monolithic}. Notably, only one study reported on the \textbf{effort} required for implementation with different web frameworks, based on developer feedback~\citeS{sunardi2019mvc}.}





%The six studies in this purpose aimed to evaluate how the architectural variables impact the performance of a software system. Three studies controlled the \textbf{workload} during profiling and comparison. For example, \citeS{sunardi2019mvc} tested 1, 100, and 500 simultaneous users for different web frameworks. Two studies compared  systems under different \textbf{use case scenarios}. For example, \citeS{haughian2016benchmarking} compared the performance of two different databases (i.e., \textit{Cassandra} and \textit{MongoDB}), under heavy-read  and heavy-write workload scenarios. \citeS{avritzer2018quantitative} examined the impact of \textbf{hardware resources} (e.g., the number of CPU cores) on performance in deployments. \citeS{sunardi2019mvc} was the only study that reported the \textbf{effort} for implementing web applications with different web frameworks, based on questionnaires involving 10 \textit{PHP} project developers.
%More specifically, three studies~\citeS{avritzer2018quantitative, zulkipli2013empirical, sunardi2019mvc} investigate the performance of their web application with different workload scenarios. These web applications vary in constructive frameworks~\citeS{sunardi2019mvc} and deployment environment~\citeS{avritzer2018quantitative, zulkipli2013empirical}. \citeS{fioravanti2016experimental, haughian2016benchmarking} compare the performance of different database systems executing the same operations. For example, in \citeS{fioravanti2016experimental}, researchers found that the \textit{NoSQL} data storage systems, \textit{MongoDB} and \textit{Neo4j}, outperforms the traditional \textit{MySQL + Hibernate} database. \citeS{lung2014measuring} compares different concurrent processing architectures, in terms of the number of threads and size of queues under different workload. 

%\lu{has this been talked about already previously? Are we repeating ourselves?} \yz{I added more details to avoid repeating ourselves.}


\textbf{d) Evaluation of the \textit{Self-Adaption} studies:} \citeS{arcelli2020multi} only conducted a case study to show the feasibility of the proposed self-adaption system. The remaining five studies evaluated the \textbf{performance improvement} achieved by the proposed self-adaption frameworks~\citeS{lung2016improving, gergin2014decentralized, camara2013evolving, camara2020quantitative, perez2010performance, ezzeddine2021design, peng2021parallel}. 
For example, \citeS{perez2010performance} achieved an average 11\% improvement in response time.
In addition, two studies measured the \textbf{return on investment} for applying the proposed self-adaption frameworks~\citeS{camara2013evolving, gergin2014decentralized}. For example, in \citeS{gergin2014decentralized}, the framework could slow down the system by 2\% to 10\% in normal conditions. However, if a burst of requests occurred, the framework could save up to 70\% time.





==> rq5.tex <==
\subsection{RQ-5: Evaluation Methodology}
\label{sec:rq5}
RQ5 examines the evaluation methodologies used in the studies. We focused on two aspects: 1) the nature and the number of evaluation subjects; and 2) the evaluation  purpose. The motivation is to provide insights for future research evaluation based on the strengths and limitations of the evaluation methods.  


\subsubsection{\textbf{Characteristics of the Evaluation Subjects}} %Figure~\ref{fig:nums-evaluating} shows the distribution of number of evaluation subjects being used in the studies. As we can see, 
First, we found that most (80\%) studies only used one evaluation subject; \textcolor{blue}{15 (14\%)} studies used two evaluation subjects;  it was rare for a study to use more than 3 evaluation subjects (just 6\%). This indicates that the general applicability of the proposed techniques is usually left untested.
 
%\begin{figure}[h]
%  \centering
%  \includegraphics[width=\columnwidth]{figures/nums-evaluating.png}  
%  \caption{Number of Evaluation Subject(s)}
%  \label{fig:nums-evaluating}
%\end{figure}

The evaluation subjects are divided into three  categories: 1) lab-based systems, which is most common in \textcolor{blue}{61} studies~\citeS{eshraghian2015performance,khan2010performance,becker2013performance,jalali2011new,barbierato2012perfbpel,geetha2011framework,litoiu2013performance,tribastone2010performance,nguyen2017parad,berardinelli2010performance,werle2020data,yasaweerasinghelage2018predicting,hauck2010automatic,kapova2010performance,trubiani2013model,etxeberria2014performance,gambi2010model,groenda2012improving,kapova2010systematic,tawhid2011automatic,naddaf2013performance,alhaj2013traceability,arcelli2013software,trubiani2020visarch,eramo2012performance,trubiani2015exploiting,li2016evaluating,mani2013propagation,von2011performance,wu2020microrca,du2015evolutionary,arcelli2019exploiting,arcelli2018performance,arcelli2015performance,trubiani2011detection,cortellessa2010digging,arcelli2017applying,arcelli2012antipattern,trubiani2014exploring,cortellessa2014approach,avritzer2018quantitative,gergin2014decentralized,perez2010performance,nalepa2015model,gaudel2011ada,hauck2011ginpex,mazkatli2020incremental,huber2016model,martens2011monolithic,sunardi2019mvc,zulkipli2013empirical,noorshams2014enriching,de2017model,gorsler2014performance,trubiani2014guilt,pinciroli2021model,chen2014detecting,trubiani2018exploiting,brosig2014quantitative, gonccalves2021monolith, blinowski2022monolithic, avritzer2020scalability, ezzeddine2021design, peng2021parallel}, 2) real-life software systems in 33 studies~\citeS{wrzosk2012applying,gomez2014performance,gribaudo2018performance,requeno2017performance,wu2015exploring,kross2017model,eismann2019integrating,gomez2018enabling,woodside2014transformation,walter2017expandable,happe2010parametric,hill2010run,brosig2014architecture,camara2013evolving,arcelli2020multi,eismann2018modeling,koziolek2011peropteryx,haughian2016benchmarking,zhao2020butterfly,fioravanti2016experimental,chen2014detecting,zhao2020performance,kwon2013mantis,camara2020quantitative,fioravanti2017engineering,trubiani2018exploiting,maddodi2020aggregate, avritzer2021multivariate, heger2013automated, pinciroli2021model, klinaku2021architecture, alzboon2022performance, ngo2022evaluating}, and 3) emulated systems in 10 studies~\citeS{brosig2014quantitative,happe2014stateful,krogmann2010using,brosig2011automated,brunnert2017continuous,arcelli2015control,wert2014automatic,wert2013supporting,lung2014measuring,lung2016improving,smith2017spe}. For the \textit{lab-based} systems, researchers implemented their system and so they have full control of the evaluation subjects. 
%There are common domains for the lab-based systems, such as \textit{E-Commerce System}~\citeS{tribastone2010performance,hauck2010automatic,kapova2010performance,gambi2010model,groenda2012improving,tawhid2011automatic,alhaj2013traceability,arcelli2013software,trubiani2020visarch,eramo2012performance,mani2013propagation,von2011performance,wu2020microrca,arcelli2019exploiting,arcelli2015performance,trubiani2011detection,cortellessa2010digging,arcelli2012antipattern,trubiani2014exploring,cortellessa2014approach,avritzer2018quantitative,hauck2011ginpex,mazkatli2020incremental,huber2016model,martens2011monolithic} and \textit{E-Health System}~\citeS{berardinelli2010performance,trubiani2013model,etxeberria2014performance,trubiani2015exploiting,pinciroli2020model}. 
%The other lab-based systems are in various domains, such as a \textit{e-Map Router} system that provides services for public transportation~\citeS{naddaf2013performance, eshraghian2015performance} and an \textit{Online Library} system for placing orders for lending and returning books in a public library~\citeS{li2016evaluating}.
For studies that used real-life projects, around one third are open source projects, such as \textit{Storm}~\citeS{requeno2017performance}, \textit{Hadoop}~\citeS{wu2015exploring, kross2017model}, \textit{Cassandra}~\citeS{kross2017model} and \textit{PDFBox}~\citeS{zhao2020butterfly, zhao2020performance} from the \textit{Apache Open Source Community}. The other two thirds are proprietary projects for more specialized domains, such as a  tax system~\citeS{hill2010run}. In 11 (12\%) studies, the systems were emulated. For example, in \citeS{arcelli2015control}, researchers used \textit{Modelica} as the emulating framework to define the physical phenomena (e.g., the number of processing units) and the workload scenarios (e.g., the number of enqueued requests). The study \citeS{lung2014measuring} adopted an emulated multi-tier system environment for experiments, where the data traffic was generated by the multiple clients with random bursts from time to time.

Finally, the evaluation subjects are in different problem domains, including E-commerce systems (39 studies), E-health systems (10 studies), data intensive systems (8 studies), and other more specific areas, such as video transcription and  E-routing systems. Unlike these traditional problem domains, four studies focus on systems with hardware and software co-design, which poses new challenges in architecture and performance modeling due to the dynamism of the physical environment~\citeS{gomez2018enabling,arcelli2020multi,smith2017spe,nguyen2017parad}. In 14 studies, the authors did not specify the problem domain but just provided general information, such as web systems~\citeS{lung2016improving, zulkipli2013empirical, arcelli2017applying} and distributed computing systems~\citeS{gribaudo2018performance}.

%E-Commerce systems are the most frequently , which manage user data and order transactions, in 39 (41\%) out of the 94 studies~\citeS{barbierato2012perfbpel,arcelli2013software,trubiani2018exploiting,happe2014stateful,hill2010run,alhaj2013traceability,arcelli2019exploiting,gambi2010model,litoiu2013performance,eramo2012performance,tawhid2011automatic,von2011performance,groenda2012improving,kapova2010performance,kapova2010systematic,gorsler2014performance,brunnert2017continuous,maddodi2020aggregate,tribastone2010performance,mani2013propagation,mazkatli2020incremental,hauck2010automatic,martens2011monolithic,avritzer2018quantitative,wert2014automatic,trubiani2011detection,arcelli2012antipattern,cortellessa2010digging,cortellessa2014approach,trubiani2014exploring,chen2014detecting,arcelli2015performance,wu2020microrca,li2016evaluating,trubiani2020visarch,huber2016model,trubiani2014guilt,brosig2014quantitative,koziolek2011peropteryx}, such as such as \textit{Book Store}~\citeS{von2011performance, wert2014automatic} and \textit{Sock Shop}~\citeS{avritzer2018quantitative, wu2020microrca, trubiani2018exploiting} which allow users to order books or socks online. 2) E-Health systems, which store and manage patients' or doctors' information in a hospital or a clinic, in 10 (11\%) studies~\citeS{woodside2014transformation,trubiani2015exploiting,trubiani2013model,berardinelli2010performance,etxeberria2014performance,fioravanti2016experimental,pinciroli2020model,walter2017expandable,fioravanti2017engineering,trubiani2014guilt}, such as \textit{Electronic Health Record} system~\citeS{fioravanti2016experimental} which is in use in a major Italian hospital. 3) Data intensive systems for data storage, transmission, and manipulation, in 8 (9\%) studies~\citeS{werle2020data,requeno2017performance,nalepa2015model,kross2017model,yasaweerasinghelage2018predicting,haughian2016benchmarking,gergin2014decentralized,gaudel2011ada}, such as the data analytic framework, \textit{Apache Spark}~\citeS{kross2017model} and the databases like \textit{Cassandra} and \textit{MongoDB}~\citeS{haughian2016benchmarking}. 4) Process control systems for controlling industrial processes (e.g., power generation, oil refinement, etc.), used in 5 (5\%) studies~\citeS{camara2013evolving, brosig2014quantitative, arcelli2015control, koziolek2011peropteryx, perez2010performance}, such as the energy management system that provides asset management support for power producing companies based on renewable energy sources (e.g., wind, solar, etc.) in \citeS{camara2013evolving}. 5) Systems with hardware and software co-design, in 4 (4\%) studies~\citeS{gomez2018enabling,arcelli2020multi,smith2017spe,nguyen2017parad}, such as the fire alert system that analyzes the data collected from a network of smoke sensors to detect fire disaster~\citeS{arcelli2020multi}. 6) Management systems for managing the staff, visitor, or equipment in a company or an organization, in 4 (4\%) studies~\citeS{camara2020quantitative,arcelli2018performance,brosig2014architecture,hauck2011ginpex}, such as the botanical garden management system that manages the visitors and plants~\citeS{arcelli2018performance} and the supply chain management system~\citeS{hauck2011ginpex}. And finally, 7) Transportation systems for locating, routing, and guiding services, used in 4 (4\%) studies~\citeS{eshraghian2015performance,naddaf2013performance,de2017model,trubiani2014guilt}, such as the \textit{E-Map Router} system that aims to find the nearest restaurant and guide the way for a user~\citeS{eshraghian2015performance,naddaf2013performance} and the \textit{Bus-on-Air} system that provides travel planning~\citeS{de2017model}.

%There are 10 (11\%) papers, each of which focuses on a very specific problem area, and does not belong the about seven problem domains~\citeS{noorshams2014enriching,wu2015exploring,geetha2011framework,becker2013performance,kwon2013mantis,eismann2018modeling,krogmann2010using,gomez2014performance,zhao2020butterfly,zhao2020performance}. For example, \citeS{krogmann2010using} uses a file sharing application, and \citeS{eismann2018modeling} uses video subtitles auto-generation and translation system. Also, the rest 14 (15\%) studies, the authors do not specify the problem domain of the evaluation subject, but just provide general information~\citeS{noorshams2014enriching,wu2015exploring,geetha2011framework,becker2013performance,kwon2013mantis,eismann2018modeling,krogmann2010using,gomez2014performance,zhao2020butterfly,zhao2020performance}, such as web systems~\citeS{lung2016improving, zulkipli2013empirical, arcelli2017applying} and distributed computing systems~\citeS{gribaudo2018performance}.


%\yz{There are 13 papers that I am not sure how to categorize, as highlighted in yellow in our data repository. We need to discuss them.} 
%\lu{The definition of the domains is unclear. The rationale of why a study belongs to a category is questionable. For example, why pdfbox is critical system?}

%Table~\ref{tbl:subject-metrics} shows the employment of different performance metrics based on different project domains. We can draw the following observations from this table: 1) The investigation of the performance metrics, including the response time, resource utilization, throughput, and processing time are quite consistent for all project domains. For example, response time is used in the majority of  project domains (from 50\% to 100\%). 2) Specific metrics, including latency and data transmission loss, are only measured in certain domains. %\textcolor{red}{Data transmission loss is only measured for distributed computation systems, and latency is only measured in health related systems and concurrent systems.}
\begin{comment}\begin{table*}[h]
%\setlength\extrarowheight{2pt}
\setlength{\tabcolsep}{8pt}
\centering
\caption{Performance Metrics Distribution by Characteristics of Evaluating System}\label{Tab1}
\begin{tabular}{@{}lllllll}   
\hline
\textbf{Subject Domain} & \textbf{Response Time} & \textbf{Resource Utilization} & \textbf{Throughput} & \textbf{Processing Time} & \textbf{Data Trans Loss} &  \textbf{Latency} \\[0.75ex] \hline\hline

Commerce   & 97\% & 63\% & 38\% & 0 & 0 & 0 \\ \hline
Critical  & 80\% & 60\% & 50\% & 0 & 10\% & 0 \\ \hline
Data Intensive  & 50\% & 40\% & 40\% & 10\% & 0 & 30\% \\ \hline
Health   & 100\% & 29\% & 43\% & 14\% & 0 & 0\%  \\ \hline
Hw/Sw Co-Design & 75\% & 25\% & 0 & 25\% & 0 & 75\% \\ \hline
\end{tabular}
\label{tbl:subject-metrics}
\end{table*}
\end{comment}

\input{rq5-aspects}

\begin{tcolorbox}[size=title, opacityfill=0.25,enhanced, breakable]
\textbf{RQ5 Summary:} The evaluation of the 104 studies typically relies on a single study subject and lab or simulated systems. Researchers are often narrowly focused on the technical effectiveness of their proposed approach, without considering practical factors, such as usability and the costs and benefits that may impact   adoption in practice. This highlights a potential limitation of existing studies in generalizability, reproducibility, and practicality. Researchers and practitioners can refer use this knowledge to identify gaps to guide future research.
\end{tcolorbox}


==> rq6.tex <==
%\subsection{RQ-6: What performance metrics are used in related studies? How are these metrics collected?}
%\label{sec:rq6}

%\textcolor{red}{Table~\ref{tbl:metrics} can be simplified. We can remove the references, and draw a histogram to show the number of studies that used each metric. We also need to change the order of the metrics based on the popularity to be more reader friendly. The same for other tables.}
%We answer this RQ based on data items, D15 and D16, from Table~\ref{tbl:annotation}. 






\begin{comment}
\begin{table*}
	\centering
	\scriptsize
	\caption{Performance Metrics Distribution by Characteristics of Evaluating System \label{tbl:domains}}{
		\resizebox{\linewidth}{!}{\begin{tabular}{|l|c|c|c|c|c|c|c|} 
				\hline
				Subject Characteristic  & Response Time & Resource Utilization & Throughput & Processing Time  & Data Transmission Loss & Latency & Power Consumption \\  \hline
				Critical System                 & 62\% & 62\% & 38\% & 31\%  & 15\% & 8\% & 15\%  \\ \hline
				E-Commerce System               & 100\% & 56\% & 44\% & 22\% & 0\%  & 0\% & 0\% \\ \hline
				Distributed Concurrent System   & 71\% & 57\% & 50\% & 21\% & 36\%   & 7\% & 7\% \\ \hline
				Data Intensive System           & 100\% & 67\% & 33\% & 33\% & 0\% & 0\% & 0\% \\ \hline
				Cloud Computing System          & 50\% & 75\% & 75\% & 25\%  & 0\%  & 25\% & 0\% \\ \hline \hline
				  
				Average                         & 77\% & 54\% & 42\% & 29\% & 13\% & 12\%  & 6\% \\ \hline
	\end{tabular}}}
	
\end{table*}
\end{comment}

%is the response time, and it is followed by the resource utilization and throughput. This findings agrees with the prior study by Jain \textit{et al.}~\cite{jain1991art}, that the three mostly-used performance metrics are response time, resource utilization, and throughput. 

%According to Jain \textit{et al.}, three most widely-used three metrics that describe performance of software system are response time, resource utilization, and throughput~\cite{jain1991art}. All of them are related to workload~\cite{seelig2006performance}. Additionally, the application response time is increased several factors such as latency~\cite{hennessy2011computer}. The following list gives a definition of frequently used metrics in the field of software performance.


\begin{comment}
\begin{table*}[h!]
\small
\setlength{\tabcolsep}{12pt}
\caption{Architectural Models}
\begin{tabulary}{\textwidth}{@{}*1{L}*3{L}@{}}
 \hline
Performance Metric & \% & Definition & Reference(s)  \\ [0.5ex] 
 \hline\hline
Response Time & 77\% & The total time it takes from when a user makes a request until they receive a response. & \cite{jalali2011new, zhang2010improving, ramana2005some, eismann2019integrating, brosig2011automated, mani2011towards, brosig2014quantitative, xu2006evaluating, pooley2010cpasa, cortellessa2012enabling, li2016evaluating, shinozaki2006performance, du2015evolutionary, balsamo2004model, babar2004comparison, eismann2018modeling, arcelli2013software, zhao2020performance, sharafi2010analytical, xenopoulos2016big, eskenazi2004analysis, ferretti2014performance, di2004compositional, ferreira2016peesos, allan2004odepack++, arcelli2015assisting, hauck2011ginpex, brosig2012modeling, arcelli2015control, groenda2012improving, trubiani2011detection, sharma2005architecture, rudzki2006performance, etxeberria2014performance, moreno2008performance, cortellessa2006software, becker2013performance, moscato2007software, trubiani2013model, arcelli2019exploiting}  \\ \midrule
Processing Time & 29\% & The amount of time a system takes to process a given request, not including the time it takes the message to get from the user to the system or the time back to the user. & \cite{brosig2011automated, brosig2014quantitative, kang2006performance, li2016evaluating, de2008rup, zhao2020performance, liu2011impact, agrawal2015source, eskenazi2004analysis, taifi2015jenergy, seelig2006performance, fioravanti2016experimental, wu2015exploring, balsamo2005performance, becker2013performance} \\ \midrule
Resource Utilization & 54\% & The utilization of hardware resources, such as CPU/GPU or cache, needed for a given workload. & \cite{zhang2010improving, eismann2019integrating, brosig2011automated, mani2011towards, brosig2014quantitative, xu2006evaluating ,pooley2010cpasa, kang2006performance, du2015evolutionary, balsamo2004model, babar2004comparison, eismann2018modeling, arcelli2013software, hill2010run, xenopoulos2016big, agrawal2015source, eskenazi2004analysis, yasaweerasinghelage2018predicting, allan2004odepack++, arcelli2015assisting, hauck2011ginpex, brosig2012modeling, arcelli2015control, trubiani2011detection, sharma2005architecture, cortellessa2006software, becker2013performance, trubiani2013model}  \\ \midrule
Throughput  & 42\% & the aggregate amount of work done in a given amount of time. &  \cite{jalali2011new, ramana2005some, eismann2019integrating, eismann2019integrating, brosig2011automated, mani2011towards, brosig2014quantitative, pooley2010cpasa, cortellessa2012enabling, du2015evolutionary, balsamo2004model, babar2004comparison, liu2011impact, ferretti2014performance, gokhale2006performance, hauck2011ginpex, brosig2012modeling, arcelli2015control, trubiani2011detection, rudzki2006performance, cortellessa2006software, trubiani2013model} \\ \midrule
Latency & 12\% & The delay incurred in communicating a message, i.e., the time the message spends ``on the wire''. & \cite{shinozaki2006performance, eskenazi2004analysis, yasaweerasinghelage2018predicting, gokhale2006performance, seelig2006performance, moscato2007software} \\ \midrule
Message/Packet Loss & 13\% & The failure of data travelling across a computer network. & \cite{zhang2010improving, xu2006evaluating, shinozaki2006performance, ferreira2016peesos, gokhale2006performance, rudzki2006performance, moscato2007software} \\ \midrule
Power Consumption & 6\% & The electric power consumed by the specific software system, e.g. mobile application. & \cite{balsamo2004model, hill2010run, taifi2015jenergy} \\
 [1ex] 
 \hline
\end{tabulary}
\label{tbl:metrics}
\end{table*}
\end{comment}




%Base on our observation, we found that the measured performance metrics are highly relevant to the Characteristics of the evaluating systems. We classified the evaluating systems in the reviewed studies into five classic characteristics, as shown in Table~\ref{tbl:domains}. The evaluating subjects that have those five characteristics do not cover all the evaluating subjects in all reviewed studies, since the rest of evaluating systems (around 30\%) are rather ad-hoc and do not have obvious domain. Also, the evaluating systems in different domains are not entirely independent from each other. For example, an E-Commerce related website can also be deployed in a server-client platform so it can also be a distributed concurrent system. 

%The critical system is a system with specific usage, such as the \textit{Bus-On-Air} system which aims to manage the transferring bus in an airport~\cite{cortellessa2012enabling}, or the \textit{Medical Imaging} system that aims to process the image in medical field~\cite{eskenazi2004analysis}. Most of the evaluated critical systems are real-life industrial standard subjects. The distribution of critical systems is very closed to the average distribution of performance metrics in all reviewed studies. We assume that reason for this phenomenon is that the goal for these subjects are unique. The comprehensive assessment of a complicated real-life software system needs to consider multiple performance metrics.

%The electronic commerce (E-Commerce) related system is a commonly used evaluating system since it has very many use case scenarios and easy to build. We found 8 of the 9 E-Commerce related evaluating system are self-build \textit{Toy Project}. Classic E-Commerce related systems are like \textit{Video Store} website in \cite{eismann2018modeling} and \cite{brosig2014quantitative}. It is noticeable that of the E-Commerce related systems measured response time. We assume that it is because the speed of websites plays an important role in the users experience of E-Commerce websites. 

%The distributed concurrent systems include both server side and client side. This domain of evaluating system appears in both real-life industrial standard subjects~\cite{xu2006evaluating, gokhale2006performance, eismann2018modeling, seabra2019rest} and self-built toy projects~\cite{fioravanti2016experimental, jalali2011new, zhang2010improving, eismann2019integrating, kang2006performance, sharafi2010analytical, liu2011impact, gokhale2006performance, becker2013performance}. There is a non-trivial part of these systems concerns the packet or message loss ratio. The quality of connections among the components is largely concerned in the assessment of distributed systems. 

%The data intensive systems are the like \textit{Cassandra}~\cite{taifi2015jenergy} and \textit{PostgreSQL}~\cite{ferretti2014performance}. We noticed that all these evaluating systems considered the response time. We assume that it is because the processing speed impacts heavily on the user experience of the data intensive systems. In comparison, the cloud computing system, like \textit{Spark}~\cite{xenopoulos2016big}, considers the resource utilization and throughput on a large scale. We assume that it is because the cloud computing systems are calculating massive data and the utilization of resource, e.g. memory and CPU, plays an important role in the cloud computing systems. 

%We also noticed that only distributed systems and critical system concerns packet loss ratio and power consumption. The measurement of loss ratio can only exist in the systems that are deployed in multiple machines. Also, the measurement of power consumption is mainly for large-scale complicated systems.



%\textcolor{red}{Can we summarize the types of metrics that can be collected by each tool?}

%Two studies that measure the websites deployed in distributed system used \textit{HTTPerf}, which The distinguishing characteristics of \textit{HTTPerf} are its robustness, which includes the ability to generate and sustain server overload, the support for the multiple protocols, and its extensibility to new workload generators and performance measurements. One of the reviewed study that evaluates the performance of a Map/Reduce application, e.g. \textit{Hadoop} used \textit{MRPerf}, which is a simulation tool to model to model Map/Reduce application performance on large clusters~\cite{shinozaki2006performance}. One study that evaluates the performance of Java applications used performance profiling tools include \textit{Java Flight Recorder}~\cite{yasaweerasinghelage2018predicting}. \textit{Java Flight Recorder} is a tool for collecting profiling data about a running Java application and it is pretty lightweight and causes almost no performance overhead, so it can be used even in heavily loaded production environments. 


